SLEEPYLAND: trust begins with fair evaluation of automatic sleep staging models

Despite advances in deep learning for automatic sleep staging, clinical adoption remains limited due to challenges in fair model evaluation, generalization across diverse datasets, model bias, and variability in human annotations. We present SLEEPYLAND, an open-source sleep staging evaluation framework designed to address these barriers. It includes more than 220'000 hours in-domain (ID) sleep recordings, and more than 84'000 hours out-of-domain (OOD) sleep recordings, spanning a broad range of ages, sleep-wake disorders, and hardware setups. We release pre-trained models based on high-performing SoA architectures and evaluate them under standardized conditions across single- and multi-channel EEG/EOG configurations. We introduce SOMNUS, an ensemble combining models across architectures and channel setups via soft voting. SOMNUS achieves robust performance across twenty-four different datasets, with macro-F1 scores between 68.7% and 87.2%, outperforming individual models in 94.9% of cases. Notably, SOMNUS surpasses previous SoA methods, even including cases where compared models were trained ID while SOMNUS treated the same data as OOD. Using a subset of the BSWR (N=6'633), we quantify model biases linked to age, gender, AHI, and PLMI, showing that while ensemble improves robustness, no model architecture consistently minimizes bias in performance and clinical markers estimation. In evaluations on OOD multi-annotated datasets (DOD-H, DOD-O), SOMNUS exceeds the best human scorer, i.e., MF1 85.2% vs 80.8% on DOD-H, and 80.2% vs 75.9% on DOD-O, better reproducing the scorer consensus than any individual expert (k = 0.89/0.85 and ACS = 0.95/0.94 for healthy/OSA cohorts). Finally, we introduce ensemble disagreement metrics - entropy and inter-model divergence based - predicting regions of scorer disagreement with ROC AUCs up to 0.828, offering a data-driven proxy for human uncertainty.

==> tables/effect_w_age_table.tex <==
\begin{tiny}
\begin{longtable}{@{\hskip 0pt}l@{\hskip 2pt}@{\hskip 0pt}l@{\hskip 6pt}|@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}|@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}|@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}|@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}|@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}}
\caption{\textbf{Effects on bias and performance metrics}. Estimated GAMLSS coefficients for different metrics across sleep staging models are shown. An asterisk (*) indicates a significant non-linear (spline) age effect.}\\
\label{tab:effects_bias_performance}\\
\toprule
\multicolumn{2}{l}{\textbf{}} & \multicolumn{4}{c}{(Intercept)} & \multicolumn{4}{c}{Age} & \multicolumn{4}{c}{Gender} & \multicolumn{4}{c}{AHI} & \multicolumn{4}{c}{PLMI} \\
\rotatebox{90}{Metric} & \rotatebox{90}{Parameter} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} \\
\midrule
\endfirsthead
\toprule
\multicolumn{2}{l}{\textbf{}} & \multicolumn{4}{c}{(Intercept)} & \multicolumn{4}{c}{Age} & \multicolumn{4}{c}{Gender} & \multicolumn{4}{c}{AHI} & \multicolumn{4}{c}{PLMI} \\
\rotatebox{90}{Metric} & \rotatebox{90}{Parameter} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} \\
\midrule
\endhead
\bottomrule
\endfoot
\multirow{4}{*}{MF1} & $\mu$ & 1.12 & 1.06 & 1.05 & 1.13 & * & * & * & * & -0.06 & -0.03 & -0.04 & -0.09 & -0.05 & -0.05 & -0.05 & -0.05 & -0.02 & -0.02 & -0.02 & -0.02 \\
 & $\sigma$ & -1.51 & -1.46 & -1.47 & -1.53 & * & * & * & * & 0.06 &  &  & 0.08 &  &  &  &  & 0.01 & 0.01 &  & 0.02 \\
 & $\nu$ & -22.54 & -22.54 & -22.54 & -21.54 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & $\tau$ & -22.63 & -22.63 & -22.63 & -21.63 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\cmidrule(lr){1-22}
\multirow{4}{*}{F1\textsubscript{W}} & $\mu$ & 1.93 & 1.93 & 1.90 & 1.90 & * & * & * & * & -0.24 & -0.23 & -0.24 & -0.24 & -0.07 & -0.06 & -0.07 & -0.07 & 0.01 & 0.01 & 0.01 & 0.01 \\
 & $\sigma$ & -0.97 & -0.98 & -0.99 & -0.96 & * & * & * & * & 0.18 & 0.20 & 0.19 & 0.17 & 0.02 & 0.01 & 0.02 & 0.03 &  &  &  &  \\
 & $\nu$ & -8.80 & -8.11 & -8.80 & -8.80 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & $\tau$ & -23.63 & -24.49 & -24.49 & -8.80 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\cmidrule(lr){1-22}
\multirow{4}{*}{F1\textsubscript{N1}} & $\mu$ & -0.28 & -0.22 & -0.26 & -0.39 & * & * & * & * &  & 0.03 & 0.03 &  & -0.03 & -0.02 & -0.02 & -0.04 & -0.02 & -0.02 & -0.01 & -0.02 \\
 & $\sigma$ & -0.75 & -0.79 & -0.83 & -0.72 & * & * & * & * & -0.05 & -0.03 & -0.04 & -0.04 &  &  &  & 0.02 &  &  &  &  \\
 & $\nu$ & -4.82 & -5.10 & -5.58 & -4.03 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & $\tau$ & -22.63 & -24.17 & -20.63 & -23.62 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\cmidrule(lr){1-22}
\multirow{4}{*}{F1\textsubscript{N2}} & $\mu$ & 1.68 & 1.59 & 1.58 & 1.67 & * & * & * & * &  & 0.04 & 0.04 &  & -0.09 & -0.09 & -0.09 & -0.09 & -0.03 & -0.03 & -0.02 & -0.04 \\
 & $\sigma$ & -1.35 & -1.31 & -1.32 & -1.36 & * & * & * & * &  &  &  &  & 0.05 & 0.05 & 0.05 & 0.06 & 0.02 & 0.01 & 0.01 & 0.03 \\
 & $\nu$ & -24.47 & -23.54 & -24.14 & -24.14 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & $\tau$ & -24.49 & -23.63 & -24.18 & -24.18 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\cmidrule(lr){1-22}
\multirow{4}{*}{F1\textsubscript{N3}} & $\mu$ & 1.03 & 0.78 & 0.76 & 1.25 & * & * & * & * & -0.14 & -0.05 & -0.09 & -0.20 & -0.03 & -0.03 & -0.03 & -0.03 & -0.02 & -0.03 & -0.03 & -0.03 \\
 & $\sigma$ & -0.34 & -0.21 & -0.22 & -0.47 & * & * & * & * & 0.10 &  &  & 0.15 & 0.02 & 0.02 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 & 0.02 \\
 & $\nu$ & -2.88 & -2.64 & -2.71 & -3.10 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & $\tau$ & -8.75 & -7.63 & -24.13 & -7.37 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\cmidrule(lr){1-22}
\multirow{4}{*}{F1\textsubscript{REM}} & $\mu$ & 2.09 & 2.03 & 2.04 & 2.00 & * & * & * & * &  &  &  &  & -0.05 & -0.04 & -0.05 & -0.04 &  &  &  &  \\
 & $\sigma$ & -0.95 & -0.91 & -0.94 & -0.85 & * & * & * & * &  & 0.05 &  & -0.04 & 0.02 & 0.01 & 0.02 & 0.01 & 0.04 & 0.04 & 0.05 & 0.04 \\
 & $\nu$ & -4.06 & -4.16 & -4.23 & -4.03 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & $\tau$ & -4.65 & -4.77 & -5.07 & -4.60 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\cmidrule(lr){1-22}
\multirow{2}{*}{TST} & $\mu$ & -9.05 & -8.11 & -8.98 & -9.96 & * & * & * & * & -1.37 & -0.99 & -1.35 & -1.84 & -1.95 & -1.69 & -1.77 & -2.28 & -0.47 &  &  & -0.50 \\
 & $\sigma$ & 2.86 & 2.88 & 2.88 & 2.88 & * & * & * & * & 0.08 & 0.10 & 0.08 & 0.10 & 0.03 & 0.02 & 0.04 & 0.04 & 0.04 & 0.04 & 0.03 & 0.04 \\
\cmidrule(lr){1-22}
\multirow{2}{*}{WASO} & $\mu$ & 5.70 & 5.52 & 5.87 & 6.23 & * & * & * & * & 1.91 & 1.73 & 1.94 & 2.22 & 1.53 & 1.24 & 1.42 & 1.77 &  &  &  &  \\
 & $\sigma$ & 2.78 & 2.82 & 2.80 & 2.77 & * & * & * & * & 0.08 & 0.09 & 0.09 & 0.10 & 0.06 & 0.05 & 0.06 & 0.07 & 0.04 & 0.03 & 0.03 & 0.04 \\
\cmidrule(lr){1-22}
\multirow{2}{*}{N1} & $\mu$ & -27.54 & -25.77 & -25.81 & -28.76 & * & * & * & * & -1.70 & -1.25 & -1.47 & -2.06 & -5.91 & -5.47 & -5.56 & -6.30 & -1.53 & -1.40 & -1.35 & -1.65 \\
 & $\sigma$ & 3.03 & 3.01 & 3.00 & 3.07 & * & * & * & * &  &  &  &  & 0.10 & 0.10 & 0.10 & 0.10 & 0.05 & 0.05 & 0.04 & 0.04 \\
\cmidrule(lr){1-22}
\multirow{2}{*}{N2} & $\mu$ & 36.55 & 43.38 & 43.47 & 22.68 & * & * & * & * & -3.77 & -5.37 & -4.34 & -1.99 & 3.68 & 3.10 & 2.99 & 4.33 & 1.09 & 0.89 & 1.01 & 1.17 \\
 & $\sigma$ & 3.39 & 3.46 & 3.45 & 3.36 & * & * & * & * &  &  & -0.03 &  & 0.05 & 0.05 & 0.05 & 0.06 & 0.01 &  & 0.01 & 0.02 \\
\cmidrule(lr){1-22}
\multirow{2}{*}{N3} & $\mu$ & -22.69 & -28.76 & -30.13 & -9.59 & * & * & * & * & 5.54 & 7.09 & 6.37 & 3.27 & 0.44 & 0.72 & 0.79 &  & 0.17 & 0.23 & 0.19 & 0.25 \\
 & $\sigma$ & 3.26 & 3.34 & 3.32 & 3.29 & * & * & * & * & -0.05 & -0.07 & -0.07 & -0.03 & -0.04 & -0.04 & -0.04 & -0.03 & 0.01 & 0.01 &  & 0.01 \\
\cmidrule(lr){1-22}
\multirow{2}{*}{REM} & $\mu$ & 4.33 & 2.60 & 3.21 & 5.61 & * & * & * & * & -0.65 &  & -0.88 & -0.73 & -0.19 &  &  & -0.27 & -0.37 & -0.32 & -0.29 & -0.42 \\
 & $\sigma$ & 2.42 & 2.43 & 2.39 & 2.47 & * & * & * & * & -0.03 & -0.03 & -0.04 & -0.04 &  &  & 0.01 & -0.01 & 0.02 & 0.02 & 0.02 & 0.02 \\
\cmidrule(lr){1-22}
\multirow{2}{*}{REML} & $\mu$ & 1.80 & -1.01 & -0.57 & 0.78 & * & * & * & * &  & 1.74 &  &  & 1.10 & 0.50 & 0.80 & 0.71 & 0.35 &  &  & 0.93 \\
 & $\sigma$ & 3.76 & 3.88 & 3.76 & 3.75 & * & * & * & * &  & -0.09 & 0.05 &  & 0.03 & 0.04 & 0.04 & 0.04 & 0.02 & 0.03 & 0.02 & 0.03 \\
\cmidrule(lr){1-22}
\multirow{2}{*}{AwH} & $\mu$ & 0.32 & 0.25 & 0.34 & 0.40 & * & * & * & * & 0.23 & 0.21 & 0.23 & 0.24 & 0.08 & 0.06 & 0.07 & 0.10 & -0.02 & -0.02 & -0.02 & -0.03 \\
 & $\sigma$ & 0.03 & 0.05 & 0.03 & 0.05 & * & * & * & * & 0.15 & 0.14 & 0.13 & 0.17 & 0.12 & 0.11 & 0.12 & 0.12 & 0.01 & 0.01 & 0.01 &  \\
\cmidrule(lr){1-22}
\multirow{2}{*}{TrH} & $\mu$ & -4.93 & -4.65 & -4.48 & -4.76 & * & * & * & * & 0.41 & 0.32 & 0.41 & 0.36 & -0.18 & -0.06 & -0.14 & -0.10 & 0.09 & 0.13 & 0.07 & 0.01 \\
 & $\sigma$ & 1.76 & 1.82 & 1.79 & 1.72 & * & * & * & * &  &  &  & 0.03 & 0.12 & 0.12 & 0.12 & 0.12 & 0.03 & 0.03 & 0.03 & 0.03 \\
\end{longtable}
\end{tiny}


==> tables/effect_w_age_table_bold_best.tex <==
% \begin{tiny}
% \begin{longtable}{@{\hskip 0pt}l@{\hskip 0pt}@{\hskip 0pt}l@{\hskip 1pt}|@{\hskip 1pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 1pt}|@{\hskip 1pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 1pt}|@{\hskip 1pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 1pt}|@{\hskip 1pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 1pt}|@{\hskip 1pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 0.5pt}@{\hskip 0.5pt}r@{\hskip 0.5pt}}
% \caption{\textbf{Effects on bias and performance metrics}. Age, gender, AHI, and PLMI modeled as predictors of bias and performance metrics for four sleep‑staging models, i.e., SOMNUS (\textbf{\textit{A}}), SOMNUS$_\text{U‑Sleep}$ (\textbf{\textit{A1}}), SOMNUS$_\text{DeepSleepNet}$ (\textbf{\textit{A2}}), and SOMNUS$_\text{SleepTransformer}$ (\textbf{\textit{A3}}) - exploiting the GAMLSS framework. Age was entered as a cubic spline; AHI, PLMI, and gender as linear terms. Effects were estimated for the location ($\mu$, expectation) and scale ($\sigma$, variability) parameters, while the inflated‑Beta shape parameters ($\nu$, $\tau$) were fixed at their intercepts. An asterisk (*) marks a significant non‑linear age effect.}\\
% \label{tab:effects_bias_performance}\\
% \toprule
% \multicolumn{2}{l}{\textbf{}} & \multicolumn{4}{c}{(Intercept)} & \multicolumn{4}{c}{Age} & \multicolumn{4}{c}{Gender} & \multicolumn{4}{c}{AHI} & \multicolumn{4}{c}{PLMI} \\
%  &  &
% \textbf{\textit{A}} & \textbf{\textit{A1}} & \textbf{\textit{A2}} & \textbf{\textit{A3}} &
% \textbf{\textit{A}} & \textbf{\textit{A1}} & \textbf{\textit{A2}} & \textbf{\textit{A3}} &
% \textbf{\textit{A}} & \textbf{\textit{A1}} & \textbf{\textit{A2}} & \textbf{\textit{A3}} &
% \textbf{\textit{A}} & \textbf{\textit{A1}} & \textbf{\textit{A2}} & \textbf{\textit{A3}} &
% \textbf{\textit{A}} & \textbf{\textit{A1}} & \textbf{\textit{A2}} & \textbf{\textit{A3}} \\
% \midrule
% \endfirsthead
% \toprule
% \multicolumn{2}{l}{\textbf{}} & \multicolumn{4}{c}{(Intercept)} & \multicolumn{4}{c}{Age} & \multicolumn{4}{c}{Gender} & \multicolumn{4}{c}{AHI} & \multicolumn{4}{c}{PLMI} \\
%  &  &
% \textbf{\textit{A}} & \textbf{\textit{A1}} & \textbf{\textit{A2}} & \textbf{\textit{A3}} &
% \textbf{\textit{A}} & \textbf{\textit{A1}} & \textbf{\textit{A2}} & \textbf{\textit{A3}} &
% \textbf{\textit{A}} & \textbf{\textit{A1}} & \textbf{\textit{A2}} & \textbf{\textit{A3}} &
% \textbf{\textit{A}} & \textbf{\textit{A1}} & \textbf{\textit{A2}} & \textbf{\textit{A3}} &
% \textbf{\textit{A}} & \textbf{\textit{A1}} & \textbf{\textit{A2}} & \textbf{\textit{A3}} \\
% \midrule
% \endhead
% \bottomrule
% \endfoot
% \multirow{4}{*}{MF1} & $\mu$ & 1.12 & 1.06 & 1.05 & \textbf{1.13} & * & * & * & * & -0.06 & \textbf{-0.03} & -0.04 & -0.09 & -0.05 & -0.05 & -0.05 & -0.05 & -0.02 & -0.02 & -0.02 & -0.02 \\
%  & $\sigma$ & -1.51 & -1.46 & -1.47 & \textbf{-1.53} & * & * & * & * & 0.06 &  &  & 0.08 &  &  &  &  & 0.01 & 0.01 &  & 0.02 \\
%  & $\nu$ & \textbf{-22.54} & \textbf{-22.54} &\textbf{ -22.54} & -21.54 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%  & $\tau$ & -22.63 & -22.63 & -22.63 & \textbf{-21.63} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \cmidrule(lr){1-22}
% \multirow{4}{*}{F1\textsubscript{W}} & $\mu$ & \textbf{1.93} & \textbf{1.93} & 1.90 & 1.90 & * & * & * & * & -0.24 & \textbf{-0.23} & -0.24 & -0.24 & -0.07 & \textbf{-0.06} & -0.07 & -0.07 & 0.01 & 0.01 & 0.01 & 0.01 \\
%  & $\sigma$ & -0.97 & -0.98 & \textbf{-0.99} & -0.96 & * & * & * & * & 0.18 & 0.20 & 0.19 & \textbf{0.17} & 0.02 & \textbf{0.01} & 0.02 & 0.03 &  &  &  &  \\
%  & $\nu$ & \textbf{-8.80} & -8.11 & \textbf{-8.80} & \textbf{-8.80} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%  & $\tau$ & -23.63 & -24.49 & -24.49 & \textbf{-8.80} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \cmidrule(lr){1-22}
% \multirow{4}{*}{F1\textsubscript{N1}} & $\mu$ & -0.28 & \textbf{-0.22} & -0.26 & -0.39 & * & * & * & * &  & 0.03 & 0.03 &  & -0.03 & \textbf{-0.02} & \textbf{-0.02} & -0.04 & -0.02 & -0.02 & \textbf{-0.01} & -0.02 \\
%  & $\sigma$ & -0.75 & -0.79 & \textbf{-0.83} & -0.72 & * & * & * & * & \textbf{-0.05} & -0.03 & -0.04 & -0.04 &  &  &  & 0.02 &  &  &  &  \\
%  & $\nu$ & -4.82 & -5.10 & \textbf{-5.58} & -4.03 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%  & $\tau$ & -22.63 & -24.17 & \textbf{-20.63} & -23.62 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \cmidrule(lr){1-22}
% \multirow{4}{*}{F1\textsubscript{N2}} & $\mu$ & \textbf{1.68} & 1.59 & 1.58 & 1.67 & * & * & * & * &  & 0.04 & 0.04 &  & -0.09 & -0.09 & -0.09 & -0.09 & -0.03 & -0.03 & \textbf{-0.02} & -0.04 \\
%  & $\sigma$ & -1.35 & -1.31 & -1.32 & \textbf{-1.36} & * & * & * & * &  &  &  &  & \textbf{0.05} & \textbf{0.05} & \textbf{0.05} & 0.06 & 0.02 & \textbf{0.01} & \textbf{0.01} & 0.03 \\
%  & $\nu$ & \textbf{-24.47} & -23.54 & -24.14 & -24.14 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%  & $\tau$ & -24.49 & \textbf{-23.63} & -24.18 & -24.18 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \cmidrule(lr){1-22}
% \multirow{4}{*}{F1\textsubscript{N3}} & $\mu$ & 1.03 & 0.78 & 0.76 & \textbf{1.25} & * & * & * & * & -0.14 & \textbf{-0.05} & -0.09 & -0.20 & -0.03 & -0.03 & -0.03 & -0.03 & \textbf{-0.02} & -0.03 & -0.03 & -0.03 \\
%  & $\sigma$ & -0.34 & -0.21 & -0.22 & \textbf{-0.47} & * & * & * & * & 0.10 &  &  & 0.15 & 0.02 & 0.02 & 0.02 & \textbf{0.01} & \textbf{0.01} & \textbf{0.01} & \textbf{0.01} & 0.02 \\
%  & $\nu$ & -2.88 & -2.64 & -2.71 & \textbf{-3.10} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%  & $\tau$ & -8.75 & -7.63 & -24.13 & \textbf{-7.37} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \cmidrule(lr){1-22}
% \multirow{4}{*}{F1\textsubscript{REM}} & $\mu$ & \textbf{2.09} & 2.03 & 2.04 & 2.00 & * & * & * & * &  &  &  &  & -0.05 & \textbf{-0.04} & -0.05 & \textbf{-0.04} &  &  &  &  \\
%  & $\sigma$ & \textbf{-0.95} & -0.91 & -0.94 & -0.85 & * & * & * & * &  & 0.05 &  & \textbf{-0.04} & 0.02 & \textbf{0.01} & 0.02 & \textbf{0.01} & \textbf{0.04} & \textbf{0.04} & 0.05 & \textbf{0.04} \\
%  & $\nu$ & -4.06 & -4.16 & \textbf{-4.23} & -4.03 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%  & $\tau$ & -4.65 & -4.77 & -5.07 & \textbf{-4.60} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \cmidrule(lr){1-22}
% \multirow{2}{*}{TST} & $\mu$ & -9.05 & \textbf{-8.11} & -8.98 & -9.96 & * & * & * & * & -1.37 & \textbf{-0.99} & -1.35 & -1.84 & -1.95 & \textbf{-1.69} & -1.77 & -2.28 & -0.47 &  &  & -0.50 \\
%  & $\sigma$ & \textbf{2.86} & 2.88 & 2.88 & 2.88 & * & * & * & * & \textbf{0.08} & 0.10 & \textbf{0.08} & 0.10 & 0.03 & \textbf{0.02} & 0.04 & 0.04 & 0.04 & 0.04 & \textbf{0.03} & 0.04 \\
% \cmidrule(lr){1-22}
% \multirow{2}{*}{WASO} & $\mu$ & 5.70 & \textbf{5.52} & 5.87 & 6.23 & * & * & * & * & 1.91 & \textbf{1.73} & 1.94 & 2.22 & 1.53 & \textbf{1.24} & 1.42 & 1.77 &  &  &  &  \\
%  & $\sigma$ & 2.78 & 2.82 & 2.80 & \textbf{2.77} & * & * & * & * & \textbf{0.08} & 0.09 & 0.09 & 0.10 & 0.06 & \textbf{0.05} & 0.06 & 0.07 & 0.04 & \textbf{0.03} & \textbf{0.03} & 0.04 \\
% \cmidrule(lr){1-22}
% \multirow{2}{*}{N1} & $\mu$ & -27.54 & \textbf{-25.77} & -25.81 & -28.76 & * & * & * & * & -1.70 & \textbf{-1.25} & -1.47 & -2.06 & -5.91 & \textbf{-5.47} & -5.56 & -6.30 & -1.53 & -1.40 & \textbf{-1.35} & -1.65 \\
%  & $\sigma$ & 3.03 & 3.01 & \textbf{3.00} & 3.07 & * & * & * & * &  &  &  &  & 0.10 & 0.10 & 0.10 & 0.10 & 0.05 & 0.05 & \textbf{0.04} & \textbf{0.04} \\
% \cmidrule(lr){1-22}
% \multirow{2}{*}{N2} & $\mu$ & 36.55 & 43.38 & 43.47 & \textbf{22.68} & * & * & * & * & -3.77 & \textbf{-5.37} & -4.34 & -1.99 & 3.68 & 3.10 & \textbf{2.99} & 4.33 & 1.09 & \textbf{0.89} & 1.01 & 1.17 \\
%  & $\sigma$ & 3.39 & 3.46 & 3.45 & \textbf{3.36} & * & * & * & * &  &  & -0.03 &  & \textbf{0.05} & \textbf{0.05} & \textbf{0.05} & 0.06 & 0.01 &  & 0.01 & 0.02 \\
% \cmidrule(lr){1-22}
% \multirow{2}{*}{N3} & $\mu$ & -22.69 & -28.76 & -30.13 & \textbf{-9.59} & * & * & * & * & 5.54 & \textbf{7.09} & 6.37 & 3.27 & 0.44 & 0.72 & \textbf{0.79} &  & 0.17 & 0.23 & 0.19 & \textbf{0.25} \\
%  & $\sigma$ & \textbf{3.26} & 3.34 & 3.32 & 3.29 & * & * & * & * & -0.05 & \textbf{-0.07} & \textbf{-0.07} & -0.03 & \textbf{-0.04} & \textbf{-0.04} & \textbf{-0.04} & -0.03 & 0.01 & 0.01 &  & 0.01 \\
% \cmidrule(lr){1-22}
% \multirow{2}{*}{REM} & $\mu$ & 4.33 & \textbf{2.60} & 3.21 & 5.61 & * & * & * & * & -0.65 &  & \textbf{-0.88} & -0.73 & -0.19 &  &  & \textbf{-0.27} & \textbf{-0.37} & -0.32 & -0.29 & -0.42 \\
%  & $\sigma$ & \textbf{2.42} & 2.43 & 2.39 & 2.47 & * & * & * & * & -0.03 & -0.03 & \textbf{-0.04} & \textbf{-0.04} &  &  & 0.01 & -0.01 & 0.02 & 0.02 & 0.02 & 0.02 \\
% \cmidrule(lr){1-22}
% \multirow{2}{*}{REML} & $\mu$ & 1.80 & -1.01 & \textbf{-0.57} & 0.78 & * & * & * & * &  & 1.74 &  &  & 1.10 & 0.50 & 0.80 & 0.71 & 0.35 &  &  & 0.93 \\
%  & $\sigma$ & 3.76 & 3.88 & 3.76 & \textbf{3.75} & * & * & * & * &  & \textbf{-0.09} & 0.05 &  & \textbf{0.03} & 0.04 & 0.04 & 0.04 & \textbf{0.02} & 0.03 & \textbf{0.02} & 0.03 \\
% \cmidrule(lr){1-22}
% \multirow{2}{*}{AwH} & $\mu$ & 0.32 & \textbf{0.25} & 0.34 & 0.40 & * & * & * & * & 0.23 & \textbf{0.21} & 0.23 & 0.24 & 0.08 & \textbf{0.06} & 0.07 & 0.10 & -0.02 & -0.02 & -0.02 & \textbf{-0.03} \\
%  & $\sigma$ & \textbf{0.03} & 0.05 & \textbf{0.03} & 0.05 & * & * & * & * & 0.15 & 0.14 & \textbf{0.13} & 0.17 & 0.12 & \textbf{0.11} & 0.12 & 0.12 & 0.01 & 0.01 & 0.01 &  \\
% \cmidrule(lr){1-22}
% \multirow{2}{*}{TrH} & $\mu$ & -4.93 & -4.65 & \textbf{-4.48} & -4.76 & * & * & * & * & \textbf{0.41} & 0.32 & \textbf{0.41} & 0.36 & -0.18 & \textbf{-0.06} & -0.14 & -0.10 & 0.09 & \textbf{0.13} & 0.07 & 0.01 \\
%  & $\sigma$ & 1.76 & 1.82 & 1.79 & \textbf{1.72} & * & * & * & * &  &  &  & 0.03 & 0.12 & 0.12 & 0.12 & 0.12 & 0.03 & 0.03 & 0.03 & 0.03 \\
% \end{longtable}
% \end{tiny}

\begin{table}[h]
\caption{\textbf{Bias on performance metrics}. Age, gender, AHI, and PLMI modeled as predictors of performance metrics for four sleep‑staging models, i.e., SOMNUS (\textbf{{E}}), SOMNUS$_\text{U‑Sleep}$ (\textbf{{E1}}), SOMNUS$_\text{DeepSleepNet}$ (\textbf{{E2}}), and SOMNUS$_\text{SleepTransformer}$ (\textbf{{E3}}) - exploiting the GAMLSS framework. Age was entered as a cubic spline; AHI, PLMI, and gender as linear terms. Bias estimated for the location ($\mu$, expectation) and scale ($\sigma$, variability) parameters, while the inflated‑Beta shape parameters ($\nu$, $\tau$) were fixed at their intercepts.\\}
\label{tab:bias_performance}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllllllllllllll}
\hline
\multicolumn{2}{l}{\textbf{}} & \multicolumn{4}{c}{\cellcolor{gray!10}\textbf{(Intercept)}} & \multicolumn{4}{c}{\textbf{Gender}} & \multicolumn{4}{c}{\cellcolor{gray!10}\textbf{AHI}} & \multicolumn{4}{c}{\textbf{PLMI}} \\
&  &
\cellcolor{gray!10}\textbf{{E}} & \cellcolor{gray!10}\textbf{{E1}} & \cellcolor{gray!10}\textbf{{E2}} & \cellcolor{gray!10}\textbf{{E3}} &
\textbf{{E}} & \textbf{{E1}} & \textbf{{E2}} & \textbf{{E3}} &
\cellcolor{gray!10}\textbf{{E}} & \cellcolor{gray!10}\textbf{{E1}} & \cellcolor{gray!10}\textbf{{E2}} & \cellcolor{gray!10}\textbf{{E3}} &
\textbf{{E}} & \textbf{{E1}} & \textbf{{E2}} & \textbf{{E3}} \\
\hline
\multirow{4}{*}{MF1} & $\mu$ & \cellcolor{gray!10}1.12 & \cellcolor{gray!10}1.06 & \cellcolor{gray!10}1.05 & \cellcolor{gray!10}\textbf{1.13}  & -0.06 & \textbf{-0.03} & -0.04 & -0.09 & \cellcolor{gray!10}-0.05 & \cellcolor{gray!10}-0.05 & \cellcolor{gray!10}-0.05 & \cellcolor{gray!10}-0.05 & -0.02 & -0.02 & -0.02 & -0.02 \\
& $\sigma$ & \cellcolor{gray!10}-1.51 & \cellcolor{gray!10}-1.46 & \cellcolor{gray!10}-1.47 & \cellcolor{gray!10}\textbf{-1.53}  & 0.06 &  &  & 0.08 & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & 0.01 & 0.01 &  & 0.02 \\
& $\nu$ & \cellcolor{gray!10}\textbf{-22.54} & \cellcolor{gray!10}\textbf{-22.54} & \cellcolor{gray!10}\textbf{ -22.54} & \cellcolor{gray!10}-21.54 &  &  &  &  & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} &  &  &  &  \\
& $\tau$ & \cellcolor{gray!10}-22.63 & \cellcolor{gray!10}-22.63 & \cellcolor{gray!10}-22.63 & \cellcolor{gray!10}\textbf{-21.63} &  &  &  &  & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} &  &  &  &  \\
\hline
\multirow{4}{*}{F1\textsubscript{W}} & $\mu$ & \cellcolor{gray!10}\textbf{1.93} & \cellcolor{gray!10}\textbf{1.93} & \cellcolor{gray!10}1.90 & \cellcolor{gray!10}1.90  & -0.24 & \textbf{-0.23} & -0.24 & -0.24 & \cellcolor{gray!10}-0.07 & \cellcolor{gray!10}\textbf{-0.06} & \cellcolor{gray!10}-0.07 & \cellcolor{gray!10}-0.07 & 0.01 & 0.01 & 0.01 & 0.01 \\
& $\sigma$ & \cellcolor{gray!10}-0.97 & \cellcolor{gray!10}-0.98 & \cellcolor{gray!10}\textbf{-0.99} & \cellcolor{gray!10}-0.96  & 0.18 & 0.20 & 0.19 & \textbf{0.17} & \cellcolor{gray!10}0.02 & \cellcolor{gray!10}\textbf{0.01} & \cellcolor{gray!10}0.02 & \cellcolor{gray!10}0.03 &  &  &  &  \\
& $\nu$ & \cellcolor{gray!10}\textbf{-8.80} & \cellcolor{gray!10}-8.11 & \cellcolor{gray!10}\textbf{-8.80} & \cellcolor{gray!10}\textbf{-8.80} &  &  &  &  & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} &  &  &  &  \\
& $\tau$ & \cellcolor{gray!10}-23.63 & \cellcolor{gray!10}-24.49 & \cellcolor{gray!10}-24.49 & \cellcolor{gray!10}\textbf{-8.80} &  &  &  &  & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} &  &  &  &  \\
\hline
\multirow{4}{*}{F1\textsubscript{N1}} & $\mu$ & \cellcolor{gray!10}-0.28 & \cellcolor{gray!10}\textbf{-0.22} & \cellcolor{gray!10}-0.26 & \cellcolor{gray!10}-0.39  &  & 0.03 & 0.03 &  & \cellcolor{gray!10}-0.03 & \cellcolor{gray!10}\textbf{-0.02} & \cellcolor{gray!10}\textbf{-0.02} & \cellcolor{gray!10}-0.04 & -0.02 & -0.02 & \textbf{-0.01} & -0.02 \\
& $\sigma$ & \cellcolor{gray!10}-0.75 & \cellcolor{gray!10}-0.79 & \cellcolor{gray!10}\textbf{-0.83} & \cellcolor{gray!10}-0.72  & \textbf{-0.05} & -0.03 & -0.04 & -0.04 & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10}0.02 &  &  &  &  \\
& $\nu$ & \cellcolor{gray!10}-4.82 & \cellcolor{gray!10}-5.10 & \cellcolor{gray!10}\textbf{-5.58} & \cellcolor{gray!10}-4.03 &  &  &  &  & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} &  &  &  &  \\
& $\tau$ & \cellcolor{gray!10}-22.63 & \cellcolor{gray!10}-24.17 & \cellcolor{gray!10}\textbf{-20.63} & \cellcolor{gray!10}-23.62 &  &  &  &  & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} &  &  &  &  \\
\hline
\multirow{4}{*}{F1\textsubscript{N2}} & $\mu$ & \cellcolor{gray!10}\textbf{1.68} & \cellcolor{gray!10}1.59 & \cellcolor{gray!10}1.58 & \cellcolor{gray!10}1.67 &  & 0.04 & 0.04 &  & \cellcolor{gray!10}-0.09 & \cellcolor{gray!10}-0.09 & \cellcolor{gray!10}-0.09 & \cellcolor{gray!10}-0.09 & -0.03 & -0.03 & \textbf{-0.02} & -0.04 \\
& $\sigma$ & \cellcolor{gray!10}-1.35 & \cellcolor{gray!10}-1.31 & \cellcolor{gray!10}-1.32 & \cellcolor{gray!10}\textbf{-1.36}  &  &  &  &  & \cellcolor{gray!10}\textbf{0.05} & \cellcolor{gray!10}\textbf{0.05} & \cellcolor{gray!10}\textbf{0.05} & \cellcolor{gray!10}0.06 & 0.02 & \textbf{0.01} & \textbf{0.01} & 0.03 \\
& $\nu$ & \cellcolor{gray!10}\textbf{-24.47} & \cellcolor{gray!10}-23.54 & \cellcolor{gray!10}-24.14 & \cellcolor{gray!10}-24.14 &  &  &  &  & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} &  &  &  &  \\
& $\tau$ & \cellcolor{gray!10}-24.49 & \cellcolor{gray!10}\textbf{-23.63} & \cellcolor{gray!10}-24.18 & \cellcolor{gray!10}-24.18 &  &  &  &  & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} &  &  &  &  \\
\hline
\multirow{4}{*}{F1\textsubscript{N3}} & $\mu$ & \cellcolor{gray!10}1.03 & \cellcolor{gray!10}0.78 & \cellcolor{gray!10}0.76 & \cellcolor{gray!10}\textbf{1.25} & -0.14 & \textbf{-0.05} & -0.09 & -0.20 & \cellcolor{gray!10}-0.03 & \cellcolor{gray!10}-0.03 & \cellcolor{gray!10}-0.03 & \cellcolor{gray!10}-0.03 & \textbf{-0.02} & -0.03 & -0.03 & -0.03 \\
& $\sigma$ & \cellcolor{gray!10}-0.34 & \cellcolor{gray!10}-0.21 & \cellcolor{gray!10}-0.22 & \cellcolor{gray!10}\textbf{-0.47}  & 0.10 &  &  & 0.15 & \cellcolor{gray!10}0.02 & \cellcolor{gray!10}0.02 & \cellcolor{gray!10}0.02 & \cellcolor{gray!10}\textbf{0.01} & \textbf{0.01} & \textbf{0.01} & \textbf{0.01} & 0.02 \\
& $\nu$ & \cellcolor{gray!10}-2.88 & \cellcolor{gray!10}-2.64 & \cellcolor{gray!10}-2.71 & \cellcolor{gray!10}\textbf{-3.10} &  &  &  &  & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} &  &  &  &  \\
& $\tau$ & \cellcolor{gray!10}-8.75 & \cellcolor{gray!10}-7.63 & \cellcolor{gray!10}-24.13 & \cellcolor{gray!10}\textbf{-7.37} &  &  &  &  & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} &  &  &  &  \\
\hline
\multirow{4}{*}{F1\textsubscript{REM}} & $\mu$ & \cellcolor{gray!10}\textbf{2.09} & \cellcolor{gray!10}2.03 & \cellcolor{gray!10}2.04 & \cellcolor{gray!10}2.00 &  &  &  &  & \cellcolor{gray!10}-0.05 & \cellcolor{gray!10}\textbf{-0.04} & \cellcolor{gray!10}-0.05 & \cellcolor{gray!10}\textbf{-0.04} &  &  &  &  \\
& $\sigma$ & \cellcolor{gray!10}\textbf{-0.95} & \cellcolor{gray!10}-0.91 & \cellcolor{gray!10}-0.94 & \cellcolor{gray!10}-0.85 &  & 0.05 &  & \textbf{-0.04} & \cellcolor{gray!10}0.02 & \cellcolor{gray!10}\textbf{0.01} & \cellcolor{gray!10}0.02 & \cellcolor{gray!10}\textbf{0.01} & \textbf{0.04} & \textbf{0.04} & 0.05 & \textbf{0.04} \\
& $\nu$ & \cellcolor{gray!10}-4.06 & \cellcolor{gray!10}-4.16 & \cellcolor{gray!10}\textbf{-4.23} & \cellcolor{gray!10}-4.03 &  &  &  &  & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} &  &  &  &  \\
& $\tau$ & \cellcolor{gray!10}-4.65 & \cellcolor{gray!10}-4.77 & \cellcolor{gray!10}-5.07 & \cellcolor{gray!10}\textbf{-4.60} &  &  &  &  & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10} &  &  &  &  \\
\hline
\end{tabular}}
\end{center}
\end{table}

\begin{table}[h]
\caption{\textbf{Bias on prediction-derived clinical markers}. Age, gender, AHI, and PLMI modeled as predictors of clinical markers for four sleep‑staging models, i.e., SOMNUS (\textbf{{E}}), SOMNUS$_\text{U‑Sleep}$ (\textbf{{E1}}), SOMNUS$_\text{DeepSleepNet}$ (\textbf{{E2}}), and SOMNUS$_\text{SleepTransformer}$ (\textbf{{E3}}) - exploiting the GAMLSS framework. Age was entered as a cubic spline; AHI, PLMI, and gender as linear terms. Bias estimated for the location ($\mu$, expectation) and scale ($\sigma$, variability) parameters.\\}
\label{tab:bias_markers}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllllllllllllll}
\hline
\multicolumn{2}{l}{\textbf{}} & \multicolumn{4}{c}{\cellcolor{gray!10}\textbf{(Intercept)}} & \multicolumn{4}{c}{\textbf{Gender}} & \multicolumn{4}{c}{\cellcolor{gray!10}\textbf{AHI}} & \multicolumn{4}{c}{\textbf{PLMI}} \\
 &  &
\cellcolor{gray!10}\textbf{{E}} & \cellcolor{gray!10}\textbf{{E1}} & \cellcolor{gray!10}\textbf{{E2}} & \cellcolor{gray!10}\textbf{{E3}} &
\textbf{{E}} & \textbf{{E1}} & \textbf{{E2}} & \textbf{{E3}} &
\cellcolor{gray!10}\textbf{{E}} & \cellcolor{gray!10}\textbf{{E1}} & \cellcolor{gray!10}\textbf{{E2}} & \cellcolor{gray!10}\textbf{{E3}} &
\textbf{{E}} & \textbf{{E1}} & \textbf{{E2}} & \textbf{{E3}} \\
\hline
\multirow{2}{*}{TST} & $\mu$ & \cellcolor{gray!10}-9.05 & \cellcolor{gray!10}\textbf{-8.11} & \cellcolor{gray!10}-8.98 & \cellcolor{gray!10}-9.96  & -1.37 & \textbf{-0.99} & -1.35 & -1.84 & \cellcolor{gray!10}-1.95 & \cellcolor{gray!10}\textbf{-1.69} & \cellcolor{gray!10}-1.77 & \cellcolor{gray!10}-2.28 & -0.47 &  &  & -0.50 \\
 & $\sigma$ & \cellcolor{gray!10}\textbf{2.86} & \cellcolor{gray!10}2.88 & \cellcolor{gray!10}2.88 & \cellcolor{gray!10}2.88  & \textbf{0.08} & 0.10 & \textbf{0.08} & 0.10 & \cellcolor{gray!10}0.03 & \cellcolor{gray!10}\textbf{0.02} & \cellcolor{gray!10}0.04 & \cellcolor{gray!10}0.04 & 0.04 & 0.04 & \textbf{0.03} & 0.04 \\
\hline
\multirow{2}{*}{WASO} & $\mu$ & \cellcolor{gray!10}5.70 & \cellcolor{gray!10}\textbf{5.52} & \cellcolor{gray!10}5.87 & \cellcolor{gray!10}6.23  & 1.91 & \textbf{1.73} & 1.94 & 2.22 & \cellcolor{gray!10}1.53 & \cellcolor{gray!10}\textbf{1.24} & \cellcolor{gray!10}1.42 & \cellcolor{gray!10}1.77 &  &  &  &  \\
 & $\sigma$ & \cellcolor{gray!10}2.78 & \cellcolor{gray!10}2.82 & \cellcolor{gray!10}2.80 & \cellcolor{gray!10}\textbf{2.77}  & \textbf{0.08} & 0.09 & 0.09 & 0.10 & \cellcolor{gray!10}0.06 & \cellcolor{gray!10}\textbf{0.05} & \cellcolor{gray!10}0.06 & \cellcolor{gray!10}0.07 & 0.04 & \textbf{0.03} & \textbf{0.03} & 0.04 \\
\hline
\multirow{2}{*}{N1} & $\mu$ & \cellcolor{gray!10}-27.54 & \cellcolor{gray!10}\textbf{-25.77} & \cellcolor{gray!10}-25.81 & \cellcolor{gray!10}-28.76  & -1.70 & \textbf{-1.25} & -1.47 & -2.06 & \cellcolor{gray!10}-5.91 & \cellcolor{gray!10}\textbf{-5.47} & \cellcolor{gray!10}-5.56 & \cellcolor{gray!10}-6.30 & -1.53 & -1.40 & \textbf{-1.35} & -1.65 \\
 & $\sigma$ & \cellcolor{gray!10}3.03 & \cellcolor{gray!10}3.01 & \cellcolor{gray!10}\textbf{3.00} & \cellcolor{gray!10}3.07  &  &  &  &  & \cellcolor{gray!10}0.10 & \cellcolor{gray!10}0.10 & \cellcolor{gray!10}0.10 & \cellcolor{gray!10}0.10 & 0.05 & 0.05 & \textbf{0.04} & \textbf{0.04} \\
\hline
\multirow{2}{*}{N2} & $\mu$ & \cellcolor{gray!10}36.55 & 4\cellcolor{gray!10}3.38 & \cellcolor{gray!10}43.47 & \cellcolor{gray!10}\textbf{22.68}  & -3.77 & \textbf{-5.37} & -4.34 & -1.99 & \cellcolor{gray!10}3.68 & \cellcolor{gray!10}3.10 & \cellcolor{gray!10}\textbf{2.99} & \cellcolor{gray!10}4.33 & 1.09 & \textbf{0.89} & 1.01 & 1.17 \\
 & $\sigma$ & \cellcolor{gray!10}3.39 & \cellcolor{gray!10}3.46 & \cellcolor{gray!10}3.45 & \cellcolor{gray!10}\textbf{3.36} &  &  & -0.03 &  & \cellcolor{gray!10}\textbf{0.05} & \cellcolor{gray!10}\textbf{0.05} & \cellcolor{gray!10}\textbf{0.05} & \cellcolor{gray!10}0.06 & 0.01 &  & 0.01 & 0.02 \\
\hline
\multirow{2}{*}{N3} & $\mu$ & \cellcolor{gray!10}-22.69 & \cellcolor{gray!10}-28.76 & \cellcolor{gray!10}-30.13 & \cellcolor{gray!10}\textbf{-9.59}  & 5.54 & \textbf{7.09} & 6.37 & 3.27 & \cellcolor{gray!10}0.44 & \cellcolor{gray!10}0.72 & \cellcolor{gray!10}\textbf{0.79} & \cellcolor{gray!10} & 0.17 & 0.23 & 0.19 & \textbf{0.25} \\
 & $\sigma$ & \cellcolor{gray!10}\textbf{3.26} & \cellcolor{gray!10}3.34 & \cellcolor{gray!10}3.32 & \cellcolor{gray!10}3.29  & -0.05 & \textbf{-0.07} & \textbf{-0.07} & -0.03 & \cellcolor{gray!10}\textbf{-0.04} & \cellcolor{gray!10}\textbf{-0.04} & \cellcolor{gray!10}\textbf{-0.04} & \cellcolor{gray!10}-0.03 & 0.01 & 0.01 &  & 0.01 \\
\hline
\multirow{2}{*}{REM} & $\mu$ & \cellcolor{gray!10}4.33 & \cellcolor{gray!10}\textbf{2.60} & \cellcolor{gray!10}3.21 & \cellcolor{gray!10}5.61  & -0.65 &  & \textbf{-0.88} & -0.73 & \cellcolor{gray!10}-0.19 & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10}\textbf{-0.27} & \textbf{-0.37} & -0.32 & -0.29 & -0.42 \\
 & $\sigma$ & \cellcolor{gray!10}\textbf{2.42} & \cellcolor{gray!10}2.43 & \cellcolor{gray!10}2.39 & \cellcolor{gray!10}2.47  & -0.03 & -0.03 & \textbf{-0.04} & \textbf{-0.04} & \cellcolor{gray!10} & \cellcolor{gray!10} & \cellcolor{gray!10}0.01 & \cellcolor{gray!10}-0.01 & 0.02 & 0.02 & 0.02 & 0.02 \\
\hline
\multirow{2}{*}{REML} & $\mu$ & \cellcolor{gray!10}1.80 & \cellcolor{gray!10}-1.01 & \cellcolor{gray!10}\textbf{-0.57} & \cellcolor{gray!10}0.78  &  & 1.74 &  &  & \cellcolor{gray!10}1.10 & \cellcolor{gray!10}0.50 & \cellcolor{gray!10}0.80 & \cellcolor{gray!10}0.71 & 0.35 &  &  & 0.93 \\
 & $\sigma$ & \cellcolor{gray!10}3.76 & \cellcolor{gray!10}3.88 & \cellcolor{gray!10}3.76 & \cellcolor{gray!10}\textbf{3.75}  &  & \textbf{-0.09} & 0.05 &  & \cellcolor{gray!10}\textbf{0.03} & \cellcolor{gray!10}0.04 & \cellcolor{gray!10}0.04 & \cellcolor{gray!10}0.04 & \textbf{0.02} & 0.03 & \textbf{0.02} & 0.03 \\
\hline
\multirow{2}{*}{AwH} & $\mu$ & \cellcolor{gray!10}0.32 & \cellcolor{gray!10}\textbf{0.25} & \cellcolor{gray!10}0.34 & \cellcolor{gray!10}0.40  & 0.23 & \textbf{0.21} & 0.23 & 0.24 & \cellcolor{gray!10}0.08 & \cellcolor{gray!10}\textbf{0.06} & \cellcolor{gray!10}0.07 & \cellcolor{gray!10}0.10 & -0.02 & -0.02 & -0.02 & \textbf{-0.03} \\
 & $\sigma$ & \cellcolor{gray!10}\textbf{0.03} & \cellcolor{gray!10}0.05 & \cellcolor{gray!10}\textbf{0.03} & \cellcolor{gray!10}0.05  & 0.15 & 0.14 & \textbf{0.13} & 0.17 & \cellcolor{gray!10}0.12 & \cellcolor{gray!10}\textbf{0.11} & \cellcolor{gray!10}0.12 & \cellcolor{gray!10}0.12 & 0.01 & 0.01 & 0.01 &  \\
\hline
\multirow{2}{*}{TrH} & $\mu$ & \cellcolor{gray!10}-4.93 & \cellcolor{gray!10}-4.65 & \cellcolor{gray!10}\textbf{-4.48} & \cellcolor{gray!10}-4.76  & \textbf{0.41} & 0.32 & \textbf{0.41} & 0.36 & \cellcolor{gray!10}-0.18 & \cellcolor{gray!10}\textbf{-0.06} & \cellcolor{gray!10}-0.14 & \cellcolor{gray!10}-0.10 & 0.09 & \textbf{0.13} & 0.07 & 0.01 \\
 & $\sigma$ & \cellcolor{gray!10}1.76 & \cellcolor{gray!10}1.82 & \cellcolor{gray!10}1.79 & \cellcolor{gray!10}\textbf{1.72}  &  &  &  & 0.03 & \cellcolor{gray!10}0.12 & \cellcolor{gray!10}0.12 & \cellcolor{gray!10}0.12 & \cellcolor{gray!10}0.12 & 0.03 & 0.03 & 0.03 & 0.03 \\
 \hline
\end{tabular}}
\end{center}
\end{table}

==> tables/effect_wo_age_table.tex <==
\begin{tiny}
\begin{longtable}{@{\hskip 0pt}l@{\hskip 2pt}@{\hskip 0pt}l@{\hskip 6pt}|@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}|@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}|@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}|@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}@{\hskip 1pt}r@{\hskip 1pt}}
\caption{\textbf{Effects on bias and performance metrics}. Estimated GAMLSS coefficients for different metrics across sleep staging models are shown. An asterisk (*) indicates a significant non-linear (spline) age effect.}\\
\toprule
\multicolumn{2}{l}{\textbf{}} & \multicolumn{4}{c}{(Intercept)} & \multicolumn{4}{c}{Gender} & \multicolumn{4}{c}{AHI} & \multicolumn{4}{c}{PLMI} \\
\rotatebox{90}{Metric} & \rotatebox{90}{Parameter} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} \\
\midrule
\endfirsthead
\toprule
\multicolumn{2}{l}{\textbf{}} & \multicolumn{4}{c}{(Intercept)} & \multicolumn{4}{c}{Gender} & \multicolumn{4}{c}{AHI} & \multicolumn{4}{c}{PLMI} \\
\rotatebox{90}{Metric} & \rotatebox{90}{Parameter} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} & \rotatebox{90}{SOMNUS} & \rotatebox{90}{U-Sleep} & \rotatebox{90}{DeepSleepNet} & \rotatebox{90}{SleepTransformer} \\
\midrule
\endhead
\bottomrule
\endfoot
\multirow{4}{*}{MF1} & $\mu$ & 1.12 & 1.06 & 1.05 & 1.13 & -0.06 & -0.03 & -0.04 & -0.09 & -0.05 & -0.05 & -0.05 & -0.05 & -0.02 & -0.02 & -0.02 & -0.02 \\
 & $\sigma$ & -1.51 & -1.46 & -1.47 & -1.53 & 0.06 &  &  & 0.08 &  &  &  &  & 0.01 & 0.01 &  & 0.02 \\
 & $\nu$ & -22.54 & -22.54 & -22.54 & -21.54 &  &  &  &  &  &  &  &  &  &  &  &  \\
 & $\tau$ & -22.63 & -22.63 & -22.63 & -21.63 &  &  &  &  &  &  &  &  &  &  &  &  \\
\cmidrule(lr){1-18}
\multirow{4}{*}{F1\textsubscript{W}} & $\mu$ & 1.93 & 1.93 & 1.90 & 1.90 & -0.24 & -0.23 & -0.24 & -0.24 & -0.07 & -0.06 & -0.07 & -0.07 & 0.01 & 0.01 & 0.01 & 0.01 \\
 & $\sigma$ & -0.97 & -0.98 & -0.99 & -0.96 & 0.18 & 0.20 & 0.19 & 0.17 & 0.02 & 0.01 & 0.02 & 0.03 &  &  &  &  \\
 & $\nu$ & -8.80 & -8.11 & -8.80 & -8.80 &  &  &  &  &  &  &  &  &  &  &  &  \\
 & $\tau$ & -23.63 & -24.49 & -24.49 & -8.80 &  &  &  &  &  &  &  &  &  &  &  &  \\
\cmidrule(lr){1-18}
\multirow{4}{*}{F1\textsubscript{N1}} & $\mu$ & -0.28 & -0.22 & -0.26 & -0.39 &  & 0.03 & 0.03 &  & -0.03 & -0.02 & -0.02 & -0.04 & -0.02 & -0.02 & -0.01 & -0.02 \\
 & $\sigma$ & -0.75 & -0.79 & -0.83 & -0.72 & -0.05 & -0.03 & -0.04 & -0.04 &  &  &  & 0.02 &  &  &  &  \\
 & $\nu$ & -4.82 & -5.10 & -5.58 & -4.03 &  &  &  &  &  &  &  &  &  &  &  &  \\
 & $\tau$ & -22.63 & -24.17 & -20.63 & -23.62 &  &  &  &  &  &  &  &  &  &  &  &  \\
\cmidrule(lr){1-18}
\multirow{4}{*}{F1\textsubscript{N2}} & $\mu$ & 1.68 & 1.59 & 1.58 & 1.67 &  & 0.04 & 0.04 &  & -0.09 & -0.09 & -0.09 & -0.09 & -0.03 & -0.03 & -0.02 & -0.04 \\
 & $\sigma$ & -1.35 & -1.31 & -1.32 & -1.36 &  &  &  &  & 0.05 & 0.05 & 0.05 & 0.06 & 0.02 & 0.01 & 0.01 & 0.03 \\
 & $\nu$ & -24.47 & -23.54 & -24.14 & -24.14 &  &  &  &  &  &  &  &  &  &  &  &  \\
 & $\tau$ & -24.49 & -23.63 & -24.18 & -24.18 &  &  &  &  &  &  &  &  &  &  &  &  \\
\cmidrule(lr){1-18}
\multirow{4}{*}{F1\textsubscript{N3}} & $\mu$ & 1.03 & 0.78 & 0.76 & 1.25 & -0.14 & -0.05 & -0.09 & -0.20 & -0.03 & -0.03 & -0.03 & -0.03 & -0.02 & -0.03 & -0.03 & -0.03 \\
 & $\sigma$ & -0.34 & -0.21 & -0.22 & -0.47 & 0.10 &  &  & 0.15 & 0.02 & 0.02 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 & 0.02 \\
 & $\nu$ & -2.88 & -2.64 & -2.71 & -3.10 &  &  &  &  &  &  &  &  &  &  &  &  \\
 & $\tau$ & -8.75 & -7.63 & -24.13 & -7.37 &  &  &  &  &  &  &  &  &  &  &  &  \\
\cmidrule(lr){1-18}
\multirow{4}{*}{F1\textsubscript{REM}} & $\mu$ & 2.09 & 2.03 & 2.04 & 2.00 &  &  &  &  & -0.05 & -0.04 & -0.05 & -0.04 &  &  &  &  \\
 & $\sigma$ & -0.95 & -0.91 & -0.94 & -0.85 &  & 0.05 &  & -0.04 & 0.02 & 0.01 & 0.02 & 0.01 & 0.04 & 0.04 & 0.05 & 0.04 \\
 & $\nu$ & -4.06 & -4.16 & -4.23 & -4.03 &  &  &  &  &  &  &  &  &  &  &  &  \\
 & $\tau$ & -4.65 & -4.77 & -5.07 & -4.60 &  &  &  &  &  &  &  &  &  &  &  &  \\
\cmidrule(lr){1-18}
\multirow{2}{*}{TST} & $\mu$ & -9.05 & -8.11 & -8.98 & -9.96 & -1.37 & -0.99 & -1.35 & -1.84 & -1.95 & -1.69 & -1.77 & -2.28 & -0.47 &  &  & -0.50 \\
 & $\sigma$ & 2.86 & 2.88 & 2.88 & 2.88 & 0.08 & 0.10 & 0.08 & 0.10 & 0.03 & 0.02 & 0.04 & 0.04 & 0.04 & 0.04 & 0.03 & 0.04 \\
\cmidrule(lr){1-18}
\multirow{2}{*}{WASO} & $\mu$ & 5.70 & 5.52 & 5.87 & 6.23 & 1.91 & 1.73 & 1.94 & 2.22 & 1.53 & 1.24 & 1.42 & 1.77 &  &  &  &  \\
 & $\sigma$ & 2.78 & 2.82 & 2.80 & 2.77 & 0.08 & 0.09 & 0.09 & 0.10 & 0.06 & 0.05 & 0.06 & 0.07 & 0.04 & 0.03 & 0.03 & 0.04 \\
\cmidrule(lr){1-18}
\multirow{2}{*}{N1} & $\mu$ & -27.54 & -25.77 & -25.81 & -28.76 & -1.70 & -1.25 & -1.47 & -2.06 & -5.91 & -5.47 & -5.56 & -6.30 & -1.53 & -1.40 & -1.35 & -1.65 \\
 & $\sigma$ & 3.03 & 3.01 & 3.00 & 3.07 &  &  &  &  & 0.10 & 0.10 & 0.10 & 0.10 & 0.05 & 0.05 & 0.04 & 0.04 \\
\cmidrule(lr){1-18}
\multirow{2}{*}{N2} & $\mu$ & 36.55 & 43.38 & 43.47 & 22.68 & -3.77 & -5.37 & -4.34 & -1.99 & 3.68 & 3.10 & 2.99 & 4.33 & 1.09 & 0.89 & 1.01 & 1.17 \\
 & $\sigma$ & 3.39 & 3.46 & 3.45 & 3.36 &  &  & -0.03 &  & 0.05 & 0.05 & 0.05 & 0.06 & 0.01 &  & 0.01 & 0.02 \\
\cmidrule(lr){1-18}
\multirow{2}{*}{N3} & $\mu$ & -22.69 & -28.76 & -30.13 & -9.59 & 5.54 & 7.09 & 6.37 & 3.27 & 0.44 & 0.72 & 0.79 &  & 0.17 & 0.23 & 0.19 & 0.25 \\
 & $\sigma$ & 3.26 & 3.34 & 3.32 & 3.29 & -0.05 & -0.07 & -0.07 & -0.03 & -0.04 & -0.04 & -0.04 & -0.03 & 0.01 & 0.01 &  & 0.01 \\
\cmidrule(lr){1-18}
\multirow{2}{*}{REM} & $\mu$ & 4.33 & 2.60 & 3.21 & 5.61 & -0.65 &  & -0.88 & -0.73 & -0.19 &  &  & -0.27 & -0.37 & -0.32 & -0.29 & -0.42 \\
 & $\sigma$ & 2.42 & 2.43 & 2.39 & 2.47 & -0.03 & -0.03 & -0.04 & -0.04 &  &  & 0.01 & -0.01 & 0.02 & 0.02 & 0.02 & 0.02 \\
\cmidrule(lr){1-18}
\multirow{2}{*}{REML} & $\mu$ & 1.80 & -1.01 & -0.57 & 0.78 &  & 1.74 &  &  & 1.10 & 0.50 & 0.80 & 0.71 & 0.35 &  &  & 0.93 \\
 & $\sigma$ & 3.76 & 3.88 & 3.76 & 3.75 &  & -0.09 & 0.05 &  & 0.03 & 0.04 & 0.04 & 0.04 & 0.02 & 0.03 & 0.02 & 0.03 \\
\cmidrule(lr){1-18}
\multirow{2}{*}{AwH} & $\mu$ & 0.32 & 0.25 & 0.34 & 0.40 & 0.23 & 0.21 & 0.23 & 0.24 & 0.08 & 0.06 & 0.07 & 0.10 & -0.02 & -0.02 & -0.02 & -0.03 \\
 & $\sigma$ & 0.03 & 0.05 & 0.03 & 0.05 & 0.15 & 0.14 & 0.13 & 0.17 & 0.12 & 0.11 & 0.12 & 0.12 & 0.01 & 0.01 & 0.01 &  \\
\cmidrule(lr){1-18}
\multirow{2}{*}{TrH} & $\mu$ & -4.93 & -4.65 & -4.48 & -4.76 & 0.41 & 0.32 & 0.41 & 0.36 & -0.18 & -0.06 & -0.14 & -0.10 & 0.09 & 0.13 & 0.07 & 0.01 \\
 & $\sigma$ & 1.76 & 1.82 & 1.79 & 1.72 &  &  &  & 0.03 & 0.12 & 0.12 & 0.12 & 0.12 & 0.03 & 0.03 & 0.03 & 0.03 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/LatREM.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for REM latency (REML) [minutes] bias}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & -155.98 & -155.98 & -88.39 & -88.39 & -49.13 & -49.13 & -5.50 & -5.50 & 38.14 & 38.14 & 77.40 & 77.40 & 144.99 & 144.99 \\
 & U-Sleep & -227.31 & -207.82 & -135.85 & -124.34 & -82.71 & -75.83 & -23.67 & -21.93 & 35.37 & 31.96 & 88.51 & 80.47 & 179.97 & 163.96 \\
 & DeepSleepNet & -202.61 & -211.68 & -122.58 & -127.57 & -76.07 & -78.70 & -24.40 & -24.40 & 27.27 & 29.90 & 73.78 & 78.77 & 153.81 & 162.88 \\
 & SleepTransformer & -138.98 & -138.98 & -79.39 & -79.39 & -44.77 & -44.77 & -6.30 & -6.30 & 32.17 & 32.17 & 66.79 & 66.79 & 126.38 & 126.38 \\
\cmidrule(lr){1-16}
25 & SOMNUS & -98.23 & -98.23 & -55.08 & -55.08 & -30.01 & -30.01 & -2.15 & -2.15 & 25.71 & 25.71 & 50.78 & 50.78 & 93.94 & 93.94 \\
 & U-Sleep & -120.57 & -108.87 & -69.21 & -61.97 & -39.36 & -34.73 & -6.20 & -4.46 & 26.97 & 25.82 & 56.81 & 53.06 & 108.18 & 99.95 \\
 & DeepSleepNet & -105.96 & -111.06 & -60.90 & -63.71 & -34.72 & -36.20 & -5.63 & -5.63 & 23.46 & 24.94 & 49.64 & 52.45 & 94.70 & 99.80 \\
 & SleepTransformer & -106.93 & -106.93 & -60.32 & -60.32 & -33.24 & -33.24 & -3.15 & -3.15 & 26.94 & 26.94 & 54.02 & 54.02 & 100.63 & 100.63 \\
\cmidrule(lr){1-16}
50 & SOMNUS & -84.14 & -84.14 & -45.44 & -45.44 & -22.95 & -22.95 & 2.03 & 2.03 & 27.02 & 27.02 & 49.50 & 49.50 & 88.21 & 88.21 \\
 & U-Sleep & -99.47 & -89.03 & -54.63 & -48.10 & -28.58 & -24.32 & 0.37 & 2.11 & 29.32 & 28.53 & 55.37 & 52.32 & 100.21 & 93.25 \\
 & DeepSleepNet & -83.64 & -87.93 & -45.72 & -48.09 & -23.69 & -24.93 & 0.79 & 0.79 & 25.27 & 26.52 & 47.30 & 49.67 & 85.22 & 89.51 \\
 & SleepTransformer & -82.79 & -82.79 & -45.26 & -45.26 & -23.45 & -23.45 & 0.78 & 0.78 & 25.01 & 25.01 & 46.82 & 46.82 & 84.35 & 84.35 \\
\cmidrule(lr){1-16}
75 & SOMNUS & -127.97 & -127.97 & -67.71 & -67.71 & -32.69 & -32.69 & 6.22 & 6.22 & 45.12 & 45.12 & 80.14 & 80.14 & 140.41 & 140.41 \\
 & U-Sleep & -135.87 & -122.00 & -73.36 & -64.93 & -37.03 & -31.77 & 3.33 & 5.07 & 43.68 & 41.91 & 80.01 & 75.06 & 142.52 & 132.13 \\
 & DeepSleepNet & -127.22 & -133.89 & -68.34 & -72.01 & -34.12 & -36.06 & 3.89 & 3.89 & 41.91 & 43.84 & 76.12 & 79.80 & 135.01 & 141.68 \\
 & SleepTransformer & -127.60 & -127.60 & -68.18 & -68.18 & -33.65 & -33.65 & 4.71 & 4.71 & 43.08 & 43.08 & 77.60 & 77.60 & 137.03 & 137.03 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/N1F1.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for F1\textsubscript{N1} [\%] performance}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & 0.06 & 0.07 & 0.20 & 0.20 & 0.28 & 0.28 & 0.38 & 0.38 & 0.49 & 0.49 & 0.59 & 0.59 & 0.75 & 0.74 \\
 & U-Sleep & 0.05 & 0.06 & 0.15 & 0.16 & 0.23 & 0.24 & 0.32 & 0.33 & 0.43 & 0.44 & 0.54 & 0.54 & 0.70 & 0.70 \\
 & DeepSleepNet & 0.11 & 0.13 & 0.23 & 0.25 & 0.31 & 0.32 & 0.41 & 0.42 & 0.52 & 0.52 & 0.61 & 0.61 & 0.75 & 0.75 \\
 & SleepTransformer & 0.00 & 0.00 & 0.17 & 0.18 & 0.26 & 0.26 & 0.36 & 0.36 & 0.48 & 0.47 & 0.58 & 0.57 & 0.74 & 0.73 \\
\cmidrule(lr){1-16}
25 & SOMNUS & 0.13 & 0.14 & 0.32 & 0.32 & 0.41 & 0.41 & 0.52 & 0.52 & 0.62 & 0.62 & 0.71 & 0.70 & 0.84 & 0.83 \\
 & U-Sleep & 0.17 & 0.18 & 0.33 & 0.34 & 0.42 & 0.43 & 0.52 & 0.52 & 0.62 & 0.62 & 0.70 & 0.70 & 0.82 & 0.82 \\
 & DeepSleepNet & 0.18 & 0.20 & 0.33 & 0.34 & 0.42 & 0.43 & 0.52 & 0.53 & 0.62 & 0.62 & 0.70 & 0.70 & 0.82 & 0.82 \\
 & SleepTransformer & 0.00 & 0.00 & 0.28 & 0.29 & 0.38 & 0.38 & 0.49 & 0.49 & 0.61 & 0.60 & 0.70 & 0.70 & 0.83 & 0.83 \\
\cmidrule(lr){1-16}
50 & SOMNUS & 0.08 & 0.09 & 0.24 & 0.24 & 0.33 & 0.33 & 0.44 & 0.44 & 0.56 & 0.55 & 0.66 & 0.65 & 0.80 & 0.79 \\
 & U-Sleep & 0.12 & 0.13 & 0.26 & 0.27 & 0.35 & 0.36 & 0.46 & 0.47 & 0.57 & 0.57 & 0.66 & 0.67 & 0.80 & 0.80 \\
 & DeepSleepNet & 0.12 & 0.13 & 0.25 & 0.26 & 0.34 & 0.35 & 0.44 & 0.45 & 0.55 & 0.55 & 0.64 & 0.65 & 0.78 & 0.78 \\
 & SleepTransformer & 0.00 & 0.00 & 0.20 & 0.21 & 0.30 & 0.30 & 0.41 & 0.41 & 0.53 & 0.53 & 0.64 & 0.63 & 0.79 & 0.78 \\
\cmidrule(lr){1-16}
75 & SOMNUS & 0.02 & 0.02 & 0.11 & 0.12 & 0.19 & 0.19 & 0.30 & 0.30 & 0.43 & 0.43 & 0.55 & 0.54 & 0.74 & 0.73 \\
 & U-Sleep & 0.03 & 0.03 & 0.13 & 0.14 & 0.21 & 0.22 & 0.33 & 0.34 & 0.47 & 0.47 & 0.59 & 0.59 & 0.78 & 0.77 \\
 & DeepSleepNet & 0.05 & 0.05 & 0.14 & 0.15 & 0.22 & 0.23 & 0.33 & 0.34 & 0.45 & 0.45 & 0.56 & 0.56 & 0.74 & 0.73 \\
 & SleepTransformer & 0.00 & 0.00 & 0.08 & 0.08 & 0.15 & 0.15 & 0.25 & 0.25 & 0.38 & 0.38 & 0.50 & 0.49 & 0.70 & 0.69 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/N1duration.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for N1 sleep duration [minutes] bias}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & -59.40 & -61.10 & -37.13 & -38.83 & -24.19 & -25.89 & -9.81 & -11.51 & 4.57 & 2.86 & 17.51 & 15.80 & 39.78 & 38.07 \\
 & U-Sleep & -62.50 & -63.75 & -39.65 & -40.90 & -26.37 & -27.62 & -11.62 & -12.87 & 3.13 & 1.88 & 16.40 & 15.16 & 39.25 & 38.01 \\
 & DeepSleepNet & -52.46 & -53.93 & -30.53 & -32.00 & -17.79 & -19.25 & -3.63 & -5.10 & 10.53 & 9.06 & 23.28 & 21.81 & 45.21 & 43.74 \\
 & SleepTransformer & -59.71 & -61.77 & -37.21 & -39.27 & -24.13 & -26.19 & -9.61 & -11.67 & 4.92 & 2.86 & 17.99 & 15.93 & 40.49 & 38.43 \\
\cmidrule(lr){1-16}
25 & SOMNUS & -60.38 & -62.09 & -41.96 & -43.66 & -31.26 & -32.96 & -19.36 & -21.06 & -7.47 & -9.17 & 3.24 & 1.54 & 21.66 & 19.96 \\
 & U-Sleep & -59.16 & -60.41 & -40.70 & -41.95 & -29.98 & -31.23 & -18.07 & -19.31 & -6.15 & -7.40 & 4.57 & 3.32 & 23.03 & 21.78 \\
 & DeepSleepNet & -57.78 & -59.25 & -39.92 & -41.38 & -29.54 & -31.00 & -18.00 & -19.47 & -6.47 & -7.94 & 3.91 & 2.44 & 21.78 & 20.31 \\
 & SleepTransformer & -62.53 & -64.58 & -43.48 & -45.54 & -32.41 & -34.47 & -20.12 & -22.18 & -7.82 & -9.88 & 3.25 & 1.19 & 22.29 & 20.23 \\
\cmidrule(lr){1-16}
50 & SOMNUS & -73.10 & -74.80 & -52.18 & -53.89 & -40.03 & -41.74 & -26.53 & -28.23 & -13.03 & -14.73 & -0.88 & -2.58 & 20.03 & 18.33 \\
 & U-Sleep & -70.24 & -71.49 & -49.87 & -51.12 & -38.03 & -39.28 & -24.88 & -26.13 & -11.73 & -12.98 & 0.11 & -1.14 & 20.48 & 19.23 \\
 & DeepSleepNet & -70.98 & -72.45 & -50.55 & -52.02 & -38.68 & -40.15 & -25.50 & -26.97 & -12.31 & -13.78 & -0.44 & -1.91 & 19.98 & 18.51 \\
 & SleepTransformer & -75.96 & -78.02 & -54.20 & -56.26 & -41.55 & -43.61 & -27.50 & -29.56 & -13.45 & -15.50 & -0.80 & -2.86 & 20.97 & 18.91 \\
\cmidrule(lr){1-16}
75 & SOMNUS & -100.40 & -102.10 & -74.08 & -75.78 & -58.78 & -60.48 & -41.79 & -43.49 & -24.79 & -26.49 & -9.49 & -11.19 & 16.83 & 15.13 \\
 & U-Sleep & -95.54 & -96.79 & -69.98 & -71.23 & -55.13 & -56.38 & -38.64 & -39.88 & -22.14 & -23.39 & -7.29 & -8.54 & 18.26 & 17.02 \\
 & DeepSleepNet & -95.38 & -96.84 & -69.49 & -70.96 & -54.45 & -55.92 & -37.74 & -39.21 & -21.03 & -22.50 & -5.99 & -7.46 & 19.90 & 18.43 \\
 & SleepTransformer & -105.41 & -107.47 & -78.01 & -80.07 & -62.10 & -64.16 & -44.42 & -46.47 & -26.73 & -28.79 & -10.82 & -12.88 & 16.57 & 14.52 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/N2F1.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for F1\textsubscript{N2} [\%] performance}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & 0.46 & 0.46 & 0.61 & 0.61 & 0.70 & 0.70 & 0.78 & 0.78 & 0.86 & 0.86 & 0.91 & 0.91 & 0.96 & 0.96 \\
 & U-Sleep & 0.42 & 0.43 & 0.58 & 0.59 & 0.67 & 0.68 & 0.76 & 0.77 & 0.84 & 0.84 & 0.89 & 0.90 & 0.96 & 0.96 \\
 & DeepSleepNet & 0.41 & 0.42 & 0.57 & 0.58 & 0.67 & 0.68 & 0.76 & 0.77 & 0.84 & 0.85 & 0.90 & 0.90 & 0.96 & 0.96 \\
 & SleepTransformer & 0.48 & 0.48 & 0.63 & 0.63 & 0.70 & 0.70 & 0.78 & 0.78 & 0.85 & 0.85 & 0.90 & 0.90 & 0.95 & 0.95 \\
\cmidrule(lr){1-16}
25 & SOMNUS & 0.70 & 0.70 & 0.79 & 0.79 & 0.84 & 0.84 & 0.88 & 0.88 & 0.92 & 0.92 & 0.94 & 0.94 & 0.97 & 0.97 \\
 & U-Sleep & 0.69 & 0.69 & 0.78 & 0.78 & 0.82 & 0.83 & 0.87 & 0.88 & 0.91 & 0.91 & 0.94 & 0.94 & 0.97 & 0.97 \\
 & DeepSleepNet & 0.68 & 0.69 & 0.77 & 0.78 & 0.82 & 0.83 & 0.87 & 0.87 & 0.91 & 0.91 & 0.93 & 0.94 & 0.97 & 0.97 \\
 & SleepTransformer & 0.71 & 0.71 & 0.80 & 0.80 & 0.84 & 0.84 & 0.89 & 0.89 & 0.92 & 0.92 & 0.94 & 0.94 & 0.97 & 0.97 \\
\cmidrule(lr){1-16}
50 & SOMNUS & 0.66 & 0.66 & 0.76 & 0.76 & 0.81 & 0.81 & 0.86 & 0.86 & 0.91 & 0.91 & 0.94 & 0.94 & 0.97 & 0.97 \\
 & U-Sleep & 0.63 & 0.64 & 0.74 & 0.75 & 0.80 & 0.80 & 0.85 & 0.86 & 0.90 & 0.90 & 0.93 & 0.93 & 0.97 & 0.97 \\
 & DeepSleepNet & 0.63 & 0.64 & 0.74 & 0.75 & 0.79 & 0.80 & 0.85 & 0.86 & 0.90 & 0.90 & 0.93 & 0.93 & 0.97 & 0.97 \\
 & SleepTransformer & 0.66 & 0.66 & 0.76 & 0.76 & 0.81 & 0.81 & 0.86 & 0.86 & 0.90 & 0.90 & 0.93 & 0.93 & 0.97 & 0.97 \\
\cmidrule(lr){1-16}
75 & SOMNUS & 0.49 & 0.49 & 0.64 & 0.64 & 0.72 & 0.72 & 0.80 & 0.80 & 0.86 & 0.86 & 0.91 & 0.91 & 0.96 & 0.96 \\
 & U-Sleep & 0.47 & 0.48 & 0.62 & 0.63 & 0.70 & 0.71 & 0.79 & 0.79 & 0.86 & 0.86 & 0.90 & 0.91 & 0.96 & 0.96 \\
 & DeepSleepNet & 0.48 & 0.49 & 0.62 & 0.63 & 0.71 & 0.71 & 0.79 & 0.80 & 0.86 & 0.86 & 0.90 & 0.91 & 0.96 & 0.96 \\
 & SleepTransformer & 0.47 & 0.47 & 0.62 & 0.62 & 0.70 & 0.70 & 0.79 & 0.79 & 0.86 & 0.86 & 0.90 & 0.90 & 0.96 & 0.96 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/N2duration.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for N2 sleep duration [minutes] bias}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & -45.74 & -49.51 & -2.58 & -6.35 & 22.50 & 18.73 & 50.36 & 46.59 & 78.23 & 74.46 & 103.30 & 99.53 & 146.47 & 142.70 \\
 & U-Sleep & -36.57 & -41.94 & 9.73 & 4.35 & 36.62 & 31.25 & 66.51 & 61.13 & 96.39 & 91.02 & 123.29 & 117.92 & 169.58 & 164.21 \\
 & DeepSleepNet & -40.47 & -41.34 & 6.21 & 3.78 & 33.33 & 30.00 & 63.47 & 59.13 & 93.60 & 88.26 & 120.73 & 114.48 & 167.41 & 159.60 \\
 & SleepTransformer & -73.10 & -75.09 & -30.14 & -32.12 & -5.17 & -7.16 & 22.56 & 20.57 & 50.30 & 48.31 & 75.26 & 73.27 & 118.22 & 116.23 \\
\cmidrule(lr){1-16}
25 & SOMNUS & -32.22 & -35.99 & -3.32 & -7.09 & 13.47 & 9.70 & 32.12 & 28.35 & 50.77 & 47.00 & 67.56 & 63.79 & 96.46 & 92.69 \\
 & U-Sleep & -30.03 & -35.40 & 0.54 & -4.83 & 18.30 & 12.93 & 38.04 & 32.66 & 57.77 & 52.40 & 75.54 & 70.16 & 106.11 & 100.73 \\
 & DeepSleepNet & -29.51 & -31.57 & 1.22 & -1.86 & 19.08 & 15.40 & 38.92 & 34.58 & 58.76 & 53.76 & 76.62 & 71.02 & 107.36 & 100.73 \\
 & SleepTransformer & -41.89 & -43.88 & -14.73 & -16.71 & 1.06 & -0.93 & 18.59 & 16.60 & 36.13 & 34.14 & 51.91 & 49.92 & 79.07 & 77.08 \\
\cmidrule(lr){1-16}
50 & SOMNUS & -30.09 & -33.86 & -1.66 & -5.43 & 14.86 & 11.09 & 33.22 & 29.45 & 51.58 & 47.81 & 68.10 & 64.33 & 96.53 & 92.76 \\
 & U-Sleep & -29.03 & -34.40 & 1.71 & -3.67 & 19.56 & 14.19 & 39.40 & 34.03 & 59.24 & 53.87 & 77.10 & 71.73 & 107.83 & 102.46 \\
 & DeepSleepNet & -27.40 & -29.47 & 3.09 & -0.00 & 20.80 & 17.12 & 40.48 & 36.14 & 60.16 & 55.16 & 77.87 & 72.28 & 108.36 & 101.75 \\
 & SleepTransformer & -40.87 & -42.86 & -13.11 & -15.10 & 3.02 & 1.03 & 20.94 & 18.96 & 38.87 & 36.88 & 55.00 & 53.01 & 82.76 & 80.77 \\
\cmidrule(lr){1-16}
75 & SOMNUS & -39.60 & -43.37 & 0.14 & -3.63 & 23.23 & 19.46 & 48.89 & 45.12 & 74.54 & 70.77 & 97.64 & 93.87 & 137.38 & 133.61 \\
 & U-Sleep & -34.93 & -40.30 & 6.57 & 1.19 & 30.68 & 25.31 & 57.47 & 52.10 & 84.26 & 78.89 & 108.37 & 103.00 & 149.87 & 144.50 \\
 & DeepSleepNet & -32.67 & -34.06 & 6.92 & 4.21 & 29.93 & 26.44 & 55.49 & 51.15 & 81.05 & 75.85 & 104.05 & 98.09 & 143.64 & 136.36 \\
 & SleepTransformer & -53.34 & -55.33 & -15.39 & -17.38 & 6.66 & 4.67 & 31.16 & 29.17 & 55.65 & 53.67 & 77.70 & 75.72 & 115.65 & 113.66 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/N3F1.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for F1\textsubscript{N3} [\%] performance}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & 0.00 & 0.00 & 0.66 & 0.62 & 0.78 & 0.75 & 0.86 & 0.84 & 0.92 & 0.91 & 0.96 & 0.95 & 0.99 & 0.99 \\
 & U-Sleep & 0.00 & 0.00 & 0.57 & 0.56 & 0.73 & 0.72 & 0.83 & 0.83 & 0.91 & 0.90 & 0.95 & 0.95 & 0.99 & 0.99 \\
 & DeepSleepNet & 0.00 & 0.00 & 0.55 & 0.53 & 0.71 & 0.69 & 0.82 & 0.80 & 0.90 & 0.89 & 0.95 & 0.94 & 0.99 & 0.98 \\
 & SleepTransformer & 0.00 & 0.00 & 0.75 & 0.70 & 0.82 & 0.79 & 0.88 & 0.86 & 0.92 & 0.91 & 0.95 & 0.94 & 0.98 & 0.98 \\
\cmidrule(lr){1-16}
25 & SOMNUS & 0.00 & 0.00 & 0.66 & 0.62 & 0.78 & 0.75 & 0.86 & 0.85 & 0.92 & 0.91 & 0.96 & 0.95 & 0.99 & 0.99 \\
 & U-Sleep & 0.00 & 0.00 & 0.57 & 0.55 & 0.72 & 0.71 & 0.83 & 0.82 & 0.90 & 0.90 & 0.95 & 0.94 & 0.99 & 0.99 \\
 & DeepSleepNet & 0.00 & 0.00 & 0.56 & 0.54 & 0.71 & 0.69 & 0.82 & 0.81 & 0.90 & 0.89 & 0.95 & 0.94 & 0.99 & 0.98 \\
 & SleepTransformer & 0.00 & 0.00 & 0.75 & 0.70 & 0.83 & 0.80 & 0.89 & 0.87 & 0.94 & 0.93 & 0.97 & 0.96 & 0.99 & 0.99 \\
\cmidrule(lr){1-16}
50 & SOMNUS & 0.00 & 0.00 & 0.32 & 0.27 & 0.54 & 0.49 & 0.74 & 0.71 & 0.87 & 0.86 & 0.95 & 0.94 & 0.99 & 0.99 \\
 & U-Sleep & 0.00 & 0.00 & 0.19 & 0.18 & 0.43 & 0.42 & 0.67 & 0.65 & 0.84 & 0.83 & 0.94 & 0.93 & 0.99 & 0.99 \\
 & DeepSleepNet & 0.00 & 0.00 & 0.21 & 0.19 & 0.44 & 0.42 & 0.66 & 0.64 & 0.84 & 0.82 & 0.93 & 0.92 & 0.99 & 0.99 \\
 & SleepTransformer & 0.00 & 0.00 & 0.41 & 0.33 & 0.61 & 0.55 & 0.78 & 0.74 & 0.90 & 0.88 & 0.96 & 0.96 & 1.00 & 1.00 \\
\cmidrule(lr){1-16}
75 & SOMNUS & 0.00 & 0.00 & 0.28 & 0.23 & 0.50 & 0.45 & 0.70 & 0.67 & 0.85 & 0.84 & 0.94 & 0.93 & 0.99 & 0.99 \\
 & U-Sleep & 0.00 & 0.00 & 0.16 & 0.15 & 0.39 & 0.37 & 0.62 & 0.60 & 0.81 & 0.79 & 0.91 & 0.91 & 0.99 & 0.99 \\
 & DeepSleepNet & 0.00 & 0.00 & 0.19 & 0.17 & 0.41 & 0.38 & 0.62 & 0.60 & 0.80 & 0.78 & 0.91 & 0.89 & 0.98 & 0.98 \\
 & SleepTransformer & 0.00 & 0.00 & 0.37 & 0.29 & 0.57 & 0.50 & 0.74 & 0.70 & 0.87 & 0.85 & 0.94 & 0.93 & 0.99 & 0.99 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/N3duration.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for N3 sleep duration [minutes] bias}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & -142.28 & -131.84 & -95.17 & -86.93 & -67.79 & -60.84 & -37.38 & -31.84 & -6.97 & -2.85 & 20.41 & 23.25 & 67.52 & 68.16 \\
 & U-Sleep & -155.47 & -140.93 & -105.75 & -94.56 & -76.86 & -67.61 & -44.76 & -37.67 & -12.66 & -7.73 & 16.23 & 19.21 & 65.95 & 65.59 \\
 & DeepSleepNet & -166.42 & -152.89 & -116.14 & -105.83 & -86.93 & -78.49 & -54.47 & -48.11 & -22.02 & -17.73 & 7.20 & 9.62 & 57.47 & 56.68 \\
 & SleepTransformer & -116.94 & -110.60 & -71.50 & -66.54 & -45.10 & -40.94 & -15.77 & -12.50 & 13.56 & 15.94 & 39.96 & 41.54 & 85.40 & 85.60 \\
\cmidrule(lr){1-16}
25 & SOMNUS & -81.66 & -73.50 & -56.47 & -49.49 & -41.83 & -35.54 & -25.57 & -20.03 & -9.31 & -4.53 & 5.32 & 9.42 & 30.51 & 33.43 \\
 & U-Sleep & -91.48 & -80.29 & -64.14 & -54.80 & -48.26 & -39.98 & -30.61 & -23.53 & -12.97 & -7.07 & 2.92 & 7.75 & 30.25 & 33.24 \\
 & DeepSleepNet & -92.74 & -82.47 & -65.29 & -56.77 & -49.34 & -41.85 & -31.62 & -25.26 & -13.90 & -8.67 & 2.05 & 6.26 & 29.50 & 31.95 \\
 & SleepTransformer & -64.72 & -59.86 & -41.33 & -37.19 & -27.75 & -24.02 & -12.65 & -9.38 & 2.44 & 5.26 & 16.03 & 18.43 & 39.41 & 41.11 \\
\cmidrule(lr){1-16}
50 & SOMNUS & -80.47 & -72.21 & -54.33 & -47.29 & -39.14 & -32.81 & -22.26 & -16.72 & -5.39 & -0.64 & 9.80 & 13.84 & 35.94 & 38.76 \\
 & U-Sleep & -91.48 & -80.12 & -63.00 & -53.56 & -46.46 & -38.13 & -28.07 & -20.99 & -9.69 & -3.84 & 6.86 & 11.59 & 35.34 & 38.15 \\
 & DeepSleepNet & -91.06 & -80.73 & -63.22 & -54.67 & -47.05 & -39.53 & -29.07 & -22.71 & -11.10 & -5.89 & 5.07 & 9.25 & 32.91 & 35.31 \\
 & SleepTransformer & -71.51 & -66.39 & -44.30 & -40.01 & -28.49 & -24.68 & -10.93 & -7.65 & 6.64 & 9.38 & 22.45 & 24.71 & 49.65 & 51.09 \\
\cmidrule(lr){1-16}
75 & SOMNUS & -84.97 & -76.35 & -55.36 & -48.13 & -38.16 & -31.73 & -19.05 & -13.51 & 0.06 & 4.71 & 17.27 & 21.11 & 46.87 & 49.33 \\
 & U-Sleep & -96.88 & -85.04 & -65.21 & -55.51 & -46.81 & -38.35 & -26.37 & -19.28 & -5.93 & -0.22 & 12.47 & 16.94 & 44.14 & 46.47 \\
 & DeepSleepNet & -96.74 & -85.98 & -65.85 & -57.06 & -47.90 & -40.26 & -27.96 & -21.60 & -8.02 & -2.93 & 9.92 & 13.87 & 40.81 & 42.78 \\
 & SleepTransformer & -75.86 & -70.37 & -43.05 & -38.56 & -23.99 & -20.07 & -2.81 & 0.46 & 18.37 & 21.00 & 37.43 & 39.48 & 70.24 & 71.29 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/REMF1.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for F1\textsubscript{REM} [\%] performance}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & 0.00 & 0.00 & 0.63 & 0.63 & 0.75 & 0.75 & 0.85 & 0.85 & 0.92 & 0.92 & 0.97 & 0.97 & 1.00 & 1.00 \\
 & U-Sleep & 0.00 & 0.00 & 0.58 & 0.57 & 0.71 & 0.70 & 0.82 & 0.82 & 0.90 & 0.91 & 0.95 & 0.96 & 1.00 & 1.00 \\
 & DeepSleepNet & 0.00 & 0.00 & 0.61 & 0.61 & 0.72 & 0.72 & 0.83 & 0.83 & 0.91 & 0.91 & 0.95 & 0.95 & 0.99 & 0.99 \\
 & SleepTransformer & 0.00 & 0.00 & 0.65 & 0.66 & 0.76 & 0.76 & 0.86 & 0.85 & 0.92 & 0.92 & 0.96 & 0.96 & 1.00 & 1.00 \\
\cmidrule(lr){1-16}
25 & SOMNUS & 0.00 & 0.00 & 0.79 & 0.79 & 0.86 & 0.86 & 0.92 & 0.92 & 0.96 & 0.96 & 0.98 & 0.98 & 1.00 & 1.00 \\
 & U-Sleep & 0.00 & 0.00 & 0.78 & 0.78 & 0.85 & 0.85 & 0.91 & 0.92 & 0.96 & 0.96 & 0.98 & 0.98 & 1.00 & 1.00 \\
 & DeepSleepNet & 0.00 & 0.00 & 0.77 & 0.77 & 0.85 & 0.85 & 0.91 & 0.91 & 0.96 & 0.96 & 0.98 & 0.98 & 1.00 & 1.00 \\
 & SleepTransformer & 0.00 & 0.00 & 0.76 & 0.77 & 0.85 & 0.85 & 0.91 & 0.91 & 0.96 & 0.96 & 0.98 & 0.98 & 1.00 & 1.00 \\
\cmidrule(lr){1-16}
50 & SOMNUS & 0.00 & 0.00 & 0.79 & 0.79 & 0.86 & 0.86 & 0.92 & 0.92 & 0.96 & 0.96 & 0.98 & 0.98 & 1.00 & 1.00 \\
 & U-Sleep & 0.00 & 0.00 & 0.78 & 0.78 & 0.86 & 0.85 & 0.92 & 0.92 & 0.96 & 0.96 & 0.98 & 0.98 & 1.00 & 1.00 \\
 & DeepSleepNet & 0.00 & 0.00 & 0.78 & 0.78 & 0.85 & 0.85 & 0.91 & 0.91 & 0.96 & 0.96 & 0.98 & 0.98 & 1.00 & 1.00 \\
 & SleepTransformer & 0.00 & 0.00 & 0.77 & 0.77 & 0.85 & 0.85 & 0.91 & 0.91 & 0.96 & 0.96 & 0.98 & 0.98 & 1.00 & 1.00 \\
\cmidrule(lr){1-16}
75 & SOMNUS & 0.00 & 0.00 & 0.65 & 0.65 & 0.78 & 0.78 & 0.89 & 0.89 & 0.95 & 0.95 & 0.98 & 0.98 & 1.00 & 1.00 \\
 & U-Sleep & 0.00 & 0.00 & 0.62 & 0.61 & 0.76 & 0.76 & 0.88 & 0.88 & 0.95 & 0.95 & 0.98 & 0.99 & 1.00 & 1.00 \\
 & DeepSleepNet & 0.00 & 0.00 & 0.66 & 0.66 & 0.78 & 0.78 & 0.88 & 0.88 & 0.95 & 0.95 & 0.98 & 0.98 & 1.00 & 1.00 \\
 & SleepTransformer & 0.00 & 0.00 & 0.60 & 0.61 & 0.75 & 0.76 & 0.88 & 0.88 & 0.95 & 0.95 & 0.99 & 0.98 & 1.00 & 1.00 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/REMduration.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for REM sleep duration [minutes] bias}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & -51.55 & -50.32 & -25.58 & -25.19 & -10.48 & -10.59 & 6.29 & 5.64 & 23.06 & 21.86 & 38.15 & 36.46 & 64.13 & 61.59 \\
 & U-Sleep & -62.98 & -61.13 & -33.29 & -32.26 & -16.03 & -15.49 & 3.14 & 3.14 & 22.31 & 21.77 & 39.57 & 38.54 & 69.26 & 67.40 \\
 & DeepSleepNet & -60.93 & -58.81 & -29.96 & -29.19 & -11.96 & -11.97 & 8.04 & 7.15 & 28.03 & 26.28 & 46.03 & 43.49 & 77.00 & 73.12 \\
 & SleepTransformer & -50.58 & -49.34 & -24.86 & -24.51 & -9.92 & -10.08 & 6.69 & 5.95 & 23.29 & 21.99 & 38.23 & 36.42 & 63.95 & 61.25 \\
\cmidrule(lr){1-16}
25 & SOMNUS & -20.24 & -20.04 & -8.58 & -8.77 & -1.81 & -2.21 & 5.72 & 5.07 & 13.25 & 12.35 & 20.02 & 18.90 & 31.68 & 30.18 \\
 & U-Sleep & -21.92 & -21.20 & -10.55 & -10.16 & -3.95 & -3.74 & 3.39 & 3.39 & 10.72 & 10.52 & 17.33 & 16.94 & 28.69 & 27.98 \\
 & DeepSleepNet & -20.91 & -20.68 & -9.40 & -9.67 & -2.71 & -3.27 & 4.72 & 3.83 & 12.15 & 10.94 & 18.83 & 17.33 & 30.34 & 28.34 \\
 & SleepTransformer & -20.70 & -20.47 & -8.22 & -8.42 & -0.97 & -1.42 & 7.09 & 6.36 & 15.15 & 14.14 & 22.40 & 21.14 & 34.88 & 33.19 \\
\cmidrule(lr){1-16}
50 & SOMNUS & -17.40 & -17.32 & -7.34 & -7.59 & -1.50 & -1.94 & 5.00 & 4.35 & 11.50 & 10.63 & 17.34 & 16.29 & 27.40 & 26.02 \\
 & U-Sleep & -19.27 & -18.64 & -9.08 & -8.73 & -3.16 & -2.97 & 3.43 & 3.43 & 10.01 & 9.82 & 15.93 & 15.58 & 26.13 & 25.49 \\
 & DeepSleepNet & -18.57 & -18.49 & -8.61 & -8.97 & -2.83 & -3.43 & 3.60 & 2.71 & 10.03 & 8.86 & 15.81 & 14.39 & 25.77 & 23.92 \\
 & SleepTransformer & -17.17 & -17.08 & -6.54 & -6.82 & -0.36 & -0.86 & 6.50 & 5.77 & 13.36 & 12.39 & 19.53 & 18.35 & 30.16 & 28.62 \\
\cmidrule(lr){1-16}
75 & SOMNUS & -32.12 & -31.68 & -17.07 & -17.12 & -8.33 & -8.67 & 1.38 & 0.73 & 11.09 & 10.13 & 19.84 & 18.58 & 34.88 & 33.14 \\
 & U-Sleep & -33.86 & -32.91 & -18.70 & -18.17 & -9.89 & -9.61 & -0.10 & -0.10 & 9.68 & 9.41 & 18.49 & 17.97 & 33.65 & 32.70 \\
 & DeepSleepNet & -31.30 & -30.81 & -17.15 & -17.28 & -8.93 & -9.41 & 0.21 & -0.68 & 9.34 & 8.06 & 17.56 & 15.92 & 31.71 & 29.45 \\
 & SleepTransformer & -32.69 & -32.22 & -16.97 & -17.04 & -7.84 & -8.22 & 2.31 & 1.58 & 12.46 & 11.38 & 21.59 & 20.20 & 37.31 & 35.38 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/TST.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for Total Sleep Time (TST) [minutes] bias}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & -42.27 & -47.97 & -19.14 & -22.90 & -5.71 & -8.33 & 9.22 & 7.85 & 24.15 & 24.04 & 37.59 & 38.60 & 60.72 & 63.67 \\
 & U-Sleep & -41.09 & -47.74 & -16.06 & -20.17 & -1.51 & -4.14 & 14.65 & 13.66 & 30.82 & 31.46 & 45.36 & 47.49 & 70.40 & 75.06 \\
 & DeepSleepNet & -41.29 & -47.33 & -14.60 & -18.54 & 0.90 & -1.81 & 18.13 & 16.78 & 35.36 & 35.36 & 50.86 & 52.09 & 77.54 & 80.88 \\
 & SleepTransformer & -49.74 & -56.89 & -26.18 & -30.95 & -12.49 & -15.87 & 2.72 & 0.88 & 17.93 & 17.63 & 31.62 & 32.70 & 55.18 & 58.65 \\
\cmidrule(lr){1-16}
25 & SOMNUS & -36.05 & -40.04 & -22.07 & -24.88 & -13.94 & -16.08 & -4.92 & -6.29 & 4.11 & 3.50 & 12.23 & 12.30 & 26.22 & 27.46 \\
 & U-Sleep & -36.95 & -41.16 & -22.72 & -25.48 & -14.45 & -16.38 & -5.27 & -6.26 & 3.92 & 3.86 & 12.19 & 12.97 & 26.42 & 28.64 \\
 & DeepSleepNet & -36.05 & -39.83 & -22.23 & -24.92 & -14.20 & -16.26 & -5.28 & -6.63 & 3.64 & 2.99 & 11.67 & 11.66 & 25.50 & 26.57 \\
 & SleepTransformer & -36.53 & -41.64 & -22.04 & -25.68 & -13.62 & -16.41 & -4.27 & -6.11 & 5.09 & 4.19 & 13.51 & 13.46 & 27.99 & 29.42 \\
\cmidrule(lr){1-16}
50 & SOMNUS & -48.26 & -52.88 & -30.93 & -34.09 & -20.85 & -23.17 & -9.66 & -11.04 & 1.53 & 1.09 & 11.60 & 12.01 & 28.93 & 30.80 \\
 & U-Sleep & -48.51 & -53.50 & -30.84 & -34.04 & -20.58 & -22.73 & -9.17 & -10.16 & 2.23 & 2.40 & 12.50 & 13.71 & 30.17 & 33.17 \\
 & DeepSleepNet & -49.11 & -53.56 & -31.51 & -34.57 & -21.29 & -23.54 & -9.93 & -11.29 & 1.43 & 0.97 & 11.65 & 12.00 & 29.25 & 30.98 \\
 & SleepTransformer & -49.00 & -54.78 & -31.52 & -35.54 & -21.37 & -24.36 & -10.09 & -11.93 & 1.19 & 0.49 & 11.35 & 11.67 & 28.82 & 30.92 \\
\cmidrule(lr){1-16}
75 & SOMNUS & -68.29 & -74.38 & -43.06 & -47.03 & -28.40 & -31.14 & -12.12 & -13.49 & 4.17 & 4.17 & 18.83 & 20.06 & 44.06 & 47.41 \\
 & U-Sleep & -66.00 & -72.70 & -40.77 & -44.90 & -26.11 & -28.75 & -9.82 & -10.81 & 6.47 & 7.13 & 21.13 & 23.28 & 46.36 & 51.08 \\
 & DeepSleepNet & -67.88 & -73.66 & -42.71 & -46.50 & -28.08 & -30.72 & -11.83 & -13.18 & 4.42 & 4.35 & 19.05 & 20.13 & 44.22 & 47.29 \\
 & SleepTransformer & -71.20 & -78.77 & -45.78 & -50.78 & -31.01 & -34.51 & -14.60 & -16.44 & 1.81 & 1.63 & 16.58 & 17.90 & 42.00 & 45.89 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/WASO.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for Wake After Sleep Onset (WASO) [minutes] bias}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & -39.27 & -40.25 & -23.74 & -23.42 & -14.71 & -13.64 & -4.69 & -2.77 & 5.34 & 8.09 & 14.36 & 17.87 & 29.89 & 34.70 \\
 & U-Sleep & -54.58 & -57.81 & -31.21 & -32.21 & -17.63 & -17.34 & -2.54 & -0.81 & 12.54 & 15.71 & 26.12 & 30.59 & 49.49 & 56.19 \\
 & DeepSleepNet & -63.31 & -66.80 & -37.31 & -38.36 & -22.20 & -21.83 & -5.41 & -3.46 & 11.38 & 14.90 & 26.49 & 31.43 & 52.50 & 59.87 \\
 & SleepTransformer & -33.07 & -34.48 & -18.32 & -18.10 & -9.76 & -8.59 & -0.24 & 1.98 & 9.28 & 12.55 & 17.85 & 22.06 & 32.60 & 38.44 \\
\cmidrule(lr){1-16}
25 & SOMNUS & -24.56 & -24.97 & -12.08 & -11.45 & -4.83 & -3.59 & 3.23 & 5.14 & 11.28 & 13.87 & 18.54 & 21.73 & 31.01 & 35.25 \\
 & U-Sleep & -23.96 & -24.83 & -11.75 & -11.45 & -4.65 & -3.67 & 3.24 & 4.97 & 11.12 & 13.61 & 18.22 & 21.38 & 30.44 & 34.76 \\
 & DeepSleepNet & -25.65 & -26.43 & -12.65 & -12.20 & -5.09 & -3.93 & 3.31 & 5.25 & 11.71 & 14.44 & 19.26 & 22.70 & 32.27 & 36.93 \\
 & SleepTransformer & -23.22 & -23.89 & -11.47 & -10.84 & -4.64 & -3.26 & 2.94 & 5.16 & 10.52 & 13.58 & 17.35 & 21.16 & 29.09 & 34.20 \\
\cmidrule(lr){1-16}
50 & SOMNUS & -30.72 & -31.90 & -14.14 & -13.93 & -4.50 & -3.49 & 6.20 & 8.12 & 16.91 & 19.72 & 26.54 & 30.16 & 43.13 & 48.13 \\
 & U-Sleep & -32.19 & -34.11 & -14.96 & -15.25 & -4.96 & -4.29 & 6.16 & 7.89 & 17.28 & 20.07 & 27.28 & 31.03 & 44.50 & 49.89 \\
 & DeepSleepNet & -30.22 & -31.73 & -13.69 & -13.65 & -4.09 & -3.15 & 6.58 & 8.52 & 17.25 & 20.19 & 26.85 & 30.70 & 43.38 & 48.78 \\
 & SleepTransformer & -30.62 & -32.49 & -14.00 & -14.03 & -4.34 & -3.31 & 6.39 & 8.61 & 17.12 & 20.52 & 26.77 & 31.24 & 43.39 & 49.70 \\
\cmidrule(lr){1-16}
75 & SOMNUS & -41.94 & -44.15 & -19.86 & -20.22 & -7.03 & -6.31 & 7.23 & 9.15 & 21.49 & 24.60 & 34.32 & 38.51 & 56.41 & 62.44 \\
 & U-Sleep & -43.59 & -46.65 & -21.03 & -21.94 & -7.92 & -7.58 & 6.64 & 8.37 & 21.20 & 24.32 & 34.31 & 38.68 & 56.87 & 63.39 \\
 & DeepSleepNet & -41.04 & -43.63 & -19.35 & -19.90 & -6.74 & -6.11 & 7.26 & 9.21 & 21.27 & 24.53 & 33.88 & 38.32 & 55.57 & 62.05 \\
 & SleepTransformer & -38.55 & -41.61 & -17.11 & -17.79 & -4.65 & -3.96 & 9.20 & 11.42 & 23.04 & 26.79 & 35.50 & 40.63 & 56.95 & 64.44 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/WF1.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for F1\textsubscript{W} [\%] performance}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & 0.53 & 0.43 & 0.71 & 0.64 & 0.80 & 0.75 & 0.88 & 0.86 & 0.94 & 0.93 & 0.97 & 0.97 & 1.00 & 1.00 \\
 & U-Sleep & 0.51 & 0.41 & 0.69 & 0.61 & 0.78 & 0.73 & 0.86 & 0.83 & 0.92 & 0.91 & 0.96 & 0.96 & 0.99 & 0.99 \\
 & DeepSleepNet & 0.49 & 0.38 & 0.67 & 0.59 & 0.76 & 0.71 & 0.85 & 0.82 & 0.92 & 0.91 & 0.96 & 0.95 & 0.99 & 0.99 \\
 & SleepTransformer & 0.53 & 0.43 & 0.71 & 0.64 & 0.80 & 0.75 & 0.88 & 0.86 & 0.94 & 0.93 & 0.97 & 0.97 & 1.00 & 0.99 \\
\cmidrule(lr){1-16}
25 & SOMNUS & 0.56 & 0.47 & 0.73 & 0.66 & 0.81 & 0.77 & 0.89 & 0.86 & 0.94 & 0.93 & 0.97 & 0.97 & 0.99 & 0.99 \\
 & U-Sleep & 0.55 & 0.46 & 0.72 & 0.65 & 0.80 & 0.76 & 0.88 & 0.86 & 0.94 & 0.93 & 0.97 & 0.96 & 0.99 & 0.99 \\
 & DeepSleepNet & 0.56 & 0.46 & 0.72 & 0.66 & 0.81 & 0.76 & 0.88 & 0.85 & 0.94 & 0.92 & 0.97 & 0.96 & 0.99 & 0.99 \\
 & SleepTransformer & 0.55 & 0.46 & 0.72 & 0.66 & 0.81 & 0.76 & 0.88 & 0.86 & 0.94 & 0.93 & 0.97 & 0.97 & 0.99 & 0.99 \\
\cmidrule(lr){1-16}
50 & SOMNUS & 0.59 & 0.50 & 0.75 & 0.69 & 0.82 & 0.78 & 0.89 & 0.87 & 0.94 & 0.93 & 0.97 & 0.97 & 0.99 & 0.99 \\
 & U-Sleep & 0.59 & 0.50 & 0.75 & 0.68 & 0.82 & 0.78 & 0.89 & 0.87 & 0.94 & 0.93 & 0.97 & 0.97 & 0.99 & 0.99 \\
 & DeepSleepNet & 0.59 & 0.50 & 0.74 & 0.68 & 0.82 & 0.78 & 0.89 & 0.86 & 0.94 & 0.93 & 0.97 & 0.96 & 0.99 & 0.99 \\
 & SleepTransformer & 0.58 & 0.49 & 0.74 & 0.68 & 0.82 & 0.77 & 0.89 & 0.86 & 0.94 & 0.93 & 0.97 & 0.96 & 0.99 & 0.99 \\
\cmidrule(lr){1-16}
75 & SOMNUS & 0.62 & 0.54 & 0.77 & 0.71 & 0.84 & 0.80 & 0.90 & 0.88 & 0.95 & 0.94 & 0.97 & 0.97 & 0.99 & 0.99 \\
 & U-Sleep & 0.63 & 0.54 & 0.77 & 0.72 & 0.84 & 0.81 & 0.91 & 0.88 & 0.95 & 0.94 & 0.97 & 0.97 & 0.99 & 0.99 \\
 & DeepSleepNet & 0.62 & 0.53 & 0.77 & 0.71 & 0.84 & 0.80 & 0.90 & 0.88 & 0.95 & 0.94 & 0.97 & 0.97 & 0.99 & 0.99 \\
 & SleepTransformer & 0.62 & 0.53 & 0.76 & 0.71 & 0.83 & 0.79 & 0.90 & 0.88 & 0.94 & 0.93 & 0.97 & 0.97 & 0.99 & 0.99 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/awakeningshourly.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for Awakenings per Hour (AwH) [N/hour] bias}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & -1.57 & -1.59 & -0.86 & -0.77 & -0.44 & -0.29 & 0.02 & 0.25 & 0.48 & 0.78 & 0.89 & 1.26 & 1.60 & 2.08 \\
 & U-Sleep & -1.80 & -1.85 & -1.00 & -0.93 & -0.54 & -0.40 & -0.03 & 0.19 & 0.49 & 0.78 & 0.95 & 1.31 & 1.74 & 2.22 \\
 & DeepSleepNet & -1.64 & -1.66 & -0.86 & -0.76 & -0.40 & -0.24 & 0.11 & 0.33 & 0.61 & 0.91 & 1.07 & 1.43 & 1.86 & 2.32 \\
 & SleepTransformer & -1.46 & -1.52 & -0.73 & -0.66 & -0.30 & -0.15 & 0.17 & 0.40 & 0.64 & 0.96 & 1.07 & 1.46 & 1.80 & 2.33 \\
\cmidrule(lr){1-16}
25 & SOMNUS & -1.59 & -1.67 & -0.70 & -0.65 & -0.18 & -0.05 & 0.39 & 0.62 & 0.96 & 1.28 & 1.48 & 1.88 & 2.37 & 2.91 \\
 & U-Sleep & -1.81 & -1.91 & -0.88 & -0.84 & -0.34 & -0.22 & 0.26 & 0.47 & 0.86 & 1.16 & 1.40 & 1.78 & 2.33 & 2.85 \\
 & DeepSleepNet & -1.60 & -1.65 & -0.69 & -0.62 & -0.17 & -0.02 & 0.42 & 0.64 & 1.00 & 1.31 & 1.53 & 1.91 & 2.43 & 2.94 \\
 & SleepTransformer & -1.56 & -1.68 & -0.66 & -0.62 & -0.14 & -0.01 & 0.44 & 0.68 & 1.02 & 1.36 & 1.54 & 1.97 & 2.44 & 3.03 \\
\cmidrule(lr){1-16}
50 & SOMNUS & -2.03 & -2.19 & -0.93 & -0.92 & -0.29 & -0.18 & 0.42 & 0.65 & 1.13 & 1.47 & 1.77 & 2.21 & 2.87 & 3.48 \\
 & U-Sleep & -2.11 & -2.27 & -1.00 & -1.00 & -0.36 & -0.25 & 0.36 & 0.57 & 1.08 & 1.40 & 1.72 & 2.14 & 2.83 & 3.42 \\
 & DeepSleepNet & -1.99 & -2.09 & -0.91 & -0.86 & -0.28 & -0.15 & 0.42 & 0.65 & 1.12 & 1.44 & 1.74 & 2.15 & 2.82 & 3.38 \\
 & SleepTransformer & -1.95 & -2.16 & -0.84 & -0.85 & -0.20 & -0.09 & 0.52 & 0.75 & 1.23 & 1.60 & 1.88 & 2.36 & 2.99 & 3.67 \\
\cmidrule(lr){1-16}
75 & SOMNUS & -2.82 & -3.04 & -1.54 & -1.56 & -0.81 & -0.71 & 0.02 & 0.24 & 0.84 & 1.19 & 1.58 & 2.05 & 2.85 & 3.52 \\
 & U-Sleep & -2.89 & -3.11 & -1.61 & -1.63 & -0.86 & -0.77 & -0.03 & 0.19 & 0.81 & 1.14 & 1.55 & 2.01 & 2.84 & 3.49 \\
 & DeepSleepNet & -2.78 & -2.95 & -1.50 & -1.49 & -0.75 & -0.63 & 0.09 & 0.31 & 0.92 & 1.26 & 1.67 & 2.11 & 2.95 & 3.58 \\
 & SleepTransformer & -2.86 & -3.15 & -1.55 & -1.61 & -0.79 & -0.71 & 0.05 & 0.29 & 0.90 & 1.28 & 1.66 & 2.18 & 2.96 & 3.72 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/meanF1.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for macro F1 (MF1) [\%] performance}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & 0.55 & 0.52 & 0.64 & 0.62 & 0.70 & 0.68 & 0.75 & 0.74 & 0.80 & 0.80 & 0.84 & 0.84 & 0.90 & 0.90 \\
 & U-Sleep & 0.49 & 0.49 & 0.60 & 0.59 & 0.66 & 0.65 & 0.72 & 0.71 & 0.78 & 0.77 & 0.82 & 0.82 & 0.89 & 0.88 \\
 & DeepSleepNet & 0.50 & 0.49 & 0.61 & 0.60 & 0.67 & 0.66 & 0.73 & 0.72 & 0.79 & 0.78 & 0.84 & 0.83 & 0.90 & 0.89 \\
 & SleepTransformer & 0.55 & 0.52 & 0.65 & 0.62 & 0.70 & 0.68 & 0.76 & 0.74 & 0.80 & 0.79 & 0.84 & 0.84 & 0.90 & 0.90 \\
\cmidrule(lr){1-16}
25 & SOMNUS & 0.63 & 0.61 & 0.72 & 0.70 & 0.76 & 0.75 & 0.81 & 0.80 & 0.85 & 0.84 & 0.88 & 0.88 & 0.93 & 0.93 \\
 & U-Sleep & 0.62 & 0.61 & 0.71 & 0.70 & 0.75 & 0.75 & 0.80 & 0.79 & 0.84 & 0.84 & 0.88 & 0.87 & 0.92 & 0.92 \\
 & DeepSleepNet & 0.61 & 0.60 & 0.70 & 0.69 & 0.75 & 0.74 & 0.80 & 0.79 & 0.84 & 0.83 & 0.87 & 0.87 & 0.92 & 0.92 \\
 & SleepTransformer & 0.64 & 0.61 & 0.72 & 0.70 & 0.77 & 0.75 & 0.81 & 0.80 & 0.85 & 0.84 & 0.89 & 0.88 & 0.93 & 0.93 \\
\cmidrule(lr){1-16}
50 & SOMNUS & 0.56 & 0.54 & 0.66 & 0.64 & 0.71 & 0.70 & 0.76 & 0.75 & 0.81 & 0.81 & 0.85 & 0.85 & 0.91 & 0.91 \\
 & U-Sleep & 0.54 & 0.53 & 0.64 & 0.63 & 0.70 & 0.69 & 0.75 & 0.75 & 0.81 & 0.80 & 0.85 & 0.84 & 0.91 & 0.90 \\
 & DeepSleepNet & 0.54 & 0.53 & 0.64 & 0.63 & 0.69 & 0.68 & 0.75 & 0.74 & 0.80 & 0.79 & 0.84 & 0.84 & 0.90 & 0.89 \\
 & SleepTransformer & 0.57 & 0.54 & 0.66 & 0.64 & 0.71 & 0.69 & 0.77 & 0.75 & 0.82 & 0.80 & 0.85 & 0.85 & 0.91 & 0.90 \\
\cmidrule(lr){1-16}
75 & SOMNUS & 0.46 & 0.44 & 0.58 & 0.56 & 0.64 & 0.63 & 0.71 & 0.70 & 0.77 & 0.77 & 0.82 & 0.82 & 0.89 & 0.89 \\
 & U-Sleep & 0.44 & 0.43 & 0.56 & 0.55 & 0.63 & 0.62 & 0.70 & 0.69 & 0.77 & 0.76 & 0.82 & 0.81 & 0.89 & 0.89 \\
 & DeepSleepNet & 0.44 & 0.43 & 0.56 & 0.55 & 0.63 & 0.62 & 0.70 & 0.69 & 0.77 & 0.76 & 0.82 & 0.81 & 0.89 & 0.89 \\
 & SleepTransformer & 0.46 & 0.43 & 0.58 & 0.55 & 0.64 & 0.62 & 0.71 & 0.69 & 0.77 & 0.76 & 0.82 & 0.81 & 0.89 & 0.88 \\
\end{longtable}
\end{tiny}


==> tables/quantile_tables/transitionshourly.tex <==
\begin{tiny}
\captionof{table}{\textbf{Quantile estimates for Transitions per Hour (TrH) [N/hour] bias}. Results stratified by age (5, 25, 50, 75 years), model, and gender (F/M), computed for AHI = 0 and PLMI = 0 settings.}
\begin{longtable}{l l |@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}|@{\hskip 2pt}r@{\hskip 2pt}@{\hskip 2pt}r@{\hskip 2pt}}
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endfirsthead
\toprule
 & \textbf{Quantiles:} & \multicolumn{2}{c@{\hskip 2pt}}{1\%} & \multicolumn{2}{c@{\hskip 2pt}}{10\%} & \multicolumn{2}{c@{\hskip 2pt}}{25\%} & \multicolumn{2}{c@{\hskip 2pt}}{50\%} & \multicolumn{2}{c@{\hskip 2pt}}{75\%} & \multicolumn{2}{c@{\hskip 2pt}}{90\%} & \multicolumn{2}{c@{\hskip 2pt}}{99\%} \\
\textbf{Age} & \textbf{Model} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{M} \\
\midrule
\endhead
\bottomrule
\endfoot
5 & SOMNUS & -9.57 & -9.16 & -6.67 & -6.26 & -4.99 & -4.58 & -3.11 & -2.70 & -1.24 & -0.83 & 0.45 & 0.86 & 3.35 & 3.76 \\
 & U-Sleep & -9.82 & -9.50 & -6.86 & -6.54 & -5.14 & -4.82 & -3.22 & -2.91 & -1.31 & -0.99 & 0.41 & 0.73 & 3.37 & 3.69 \\
 & DeepSleepNet & -8.77 & -8.36 & -5.64 & -5.23 & -3.82 & -3.41 & -1.80 & -1.39 & 0.22 & 0.63 & 2.04 & 2.45 & 5.17 & 5.59 \\
 & SleepTransformer & -9.77 & -9.62 & -6.63 & -6.39 & -4.81 & -4.51 & -2.78 & -2.42 & -0.76 & -0.33 & 1.07 & 1.55 & 4.21 & 4.78 \\
\cmidrule(lr){1-16}
25 & SOMNUS & -14.58 & -14.17 & -10.44 & -10.03 & -8.04 & -7.63 & -5.37 & -4.96 & -2.69 & -2.28 & -0.29 & 0.12 & 3.85 & 4.26 \\
 & U-Sleep & -14.58 & -14.26 & -10.47 & -10.15 & -8.08 & -7.77 & -5.43 & -5.11 & -2.78 & -2.46 & -0.39 & -0.07 & 3.72 & 4.04 \\
 & DeepSleepNet & -14.09 & -13.68 & -10.00 & -9.59 & -7.63 & -7.21 & -4.99 & -4.57 & -2.35 & -1.93 & 0.03 & 0.44 & 4.12 & 4.53 \\
 & SleepTransformer & -14.05 & -13.97 & -9.92 & -9.71 & -7.51 & -7.23 & -4.84 & -4.48 & -2.17 & -1.72 & 0.24 & 0.75 & 4.37 & 5.02 \\
\cmidrule(lr){1-16}
50 & SOMNUS & -19.24 & -18.83 & -13.01 & -12.60 & -9.39 & -8.98 & -5.37 & -4.96 & -1.35 & -0.94 & 2.27 & 2.68 & 8.50 & 8.91 \\
 & U-Sleep & -20.05 & -19.73 & -13.28 & -12.96 & -9.35 & -9.03 & -4.98 & -4.66 & -0.61 & -0.29 & 3.33 & 3.64 & 10.10 & 10.41 \\
 & DeepSleepNet & -19.47 & -19.06 & -12.92 & -12.51 & -9.11 & -8.70 & -4.89 & -4.47 & -0.66 & -0.24 & 3.15 & 3.56 & 9.70 & 10.11 \\
 & SleepTransformer & -18.09 & -18.12 & -12.24 & -12.10 & -8.85 & -8.60 & -5.07 & -4.71 & -1.30 & -0.82 & 2.09 & 2.68 & 7.94 & 8.70 \\
\cmidrule(lr){1-16}
75 & SOMNUS & -22.04 & -21.63 & -13.83 & -13.42 & -9.06 & -8.65 & -3.76 & -3.35 & 1.54 & 1.95 & 6.31 & 6.73 & 14.53 & 14.94 \\
 & U-Sleep & -22.33 & -22.01 & -13.99 & -13.67 & -9.14 & -8.82 & -3.75 & -3.44 & 1.63 & 1.95 & 6.48 & 6.80 & 14.82 & 15.14 \\
 & DeepSleepNet & -21.81 & -21.40 & -13.54 & -13.13 & -8.73 & -8.32 & -3.39 & -2.98 & 1.95 & 2.36 & 6.76 & 7.17 & 15.03 & 15.45 \\
 & SleepTransformer & -22.36 & -22.56 & -14.11 & -14.05 & -9.31 & -9.11 & -3.99 & -3.63 & 1.34 & 1.86 & 6.13 & 6.80 & 14.38 & 15.31 \\
\end{longtable}
\end{tiny}

